An Empirical Study of Challenges in Machine Learning Asset Management

In machine learning (ML), efficient asset management, including ML models, datasets, algorithms, and tools, is vital for resource optimization, consistent performance, and a streamlined development lifecycle. This enables quicker iterations, adaptability, reduced development-to-deployment time, and reliable outputs. Despite existing research, a significant knowledge gap remains in operational challenges like model versioning, data traceability, and collaboration, which are crucial for the success of ML projects. Our study aims to address this gap by analyzing 15,065 posts from developer forums and platforms, employing a mixed-method approach to classify inquiries, extract challenges using BERTopic, and identify solutions through open card sorting and BERTopic clustering. We uncover 133 topics related to asset management challenges, grouped into 16 macro-topics, with software dependency, model deployment, and model training being the most discussed. We also find 79 solution topics, categorized under 18 macro-topics, highlighting software dependency, feature development, and file management as key solutions. This research underscores the need for further exploration of identified pain points and the importance of collaborative efforts across academia, industry, and the research community.

==> sections/discarded.tex <==
% \begin{table}
% \centering
% \caption{Selected sample post links for solution macro-topics.}
% \begin{tabular}{ll}
% \toprule
% Example ID & Post Link \\ 
% \midrule
% $E_{01}$ & \url{https://stackoverflow.com/questions/71255132}\\
% $E_{02}$ & \url{https://stackoverflow.com/questions/70335823}\\
% $E_{03}$ & \url{https://stackoverflow.com/questions/71398882}\\
% $E_{04}$ & \url{https://stackoverflow.com/questions/72106030}\\
% $E_{05}$ & \url{https://stackoverflow.com/questions/56024351}\\
% $E_{06}$ & \url{https://github.com/getindata/kedro-kubeflow/issues/105}\\
% $E_{07}$ & \url{https://github.com/Lightning-AI/lightning/issues/6745}\\
% $E_{08}$ & \url{https://stackoverflow.com/questions/57126765}\\
% $E_{09}$ & \url{https://stackoverflow.com/questions/73811793}\\
% $E_{10}$ & \url{https://github.com/MicrosoftDocs/pipelines-azureml/issues/12}\\
% $E_{11}$ & \url{https://stackoverflow.com/questions/72068059}\\
% $E_{12}$ & \url{https://stackoverflow.com/questions/58802366}\\
% $E_{13}$ & \url{https://stackoverflow.com/questions/67258917}\\
% $E_{14}$ & \url{https://stackoverflow.com/questions/72203674}\\
% $E_{15}$ & \url{https://stackoverflow.com/questions/74406041}\\
% $E_{16}$ & \url{https://community.wandb.ai/t/vega-code/4605}\\
% $E_{17}$ & \url{https://stackoverflow.com/questions/72408785}\\
% $E_{18}$ & \url{https://stackoverflow.com/questions/73435172}\\
% \bottomrule
% \end{tabular}
% \label{rq2:post links}
% \end{table}


%By analyzing the posts without tracing its evolution, there exists a potential risk of overlooking the most recent trends or challenges. Consequently, the implications might not accurately capture the latest challenge and support patterns in the ML asset management domain. Nevertheless, we cross-reference our findings with the most recent literature in the field, ensuring that our insights are in line with current understandings.

% \begin{table}
% \centering
% \caption{Selected sample post links for challenge macro-topics.}
% \begin{tabular}{ll}
% \toprule
% Example ID & Post Link \\ 
% \midrule
% $E_{01}$ & \\
% $E_{02}$ & \url{https://stackoverflow.com/questions/75047065}\\
% $E_{03}$ & \url{https://github.com/Azure/azureml-examples/issues/242}\\
% $E_{04}$ & \url{https://github.com/aws/amazon-sagemaker-examples/issues/698}\\
% $E_{05}$ & \url{https://github.com/aws-samples/sagemaker-ssh-helper/issues/28}\\
% $E_{06}$ & \url{https://stackoverflow.com/questions/50441181}\\
% $E_{07}$ & \url{https://stackoverflow.com/questions/60088889}\\
% $E_{08}$ & \url{https://stackoverflow.com/questions/56269391}\\
% $E_{09}$ & \url{https://github.com/huggingface/transformers/issues/13111}\\
% $E_{10}$ & \url{https://github.com/aws/amazon-sagemaker-examples/issues/670}\\
% $E_{11}$ & \url{https://stackoverflow.com/questions/74257398}\\
% $E_{12}$ & \url{https://github.com/allegroai/clearml-server/issues/201}\\
% $E_{13}$ & \url{https://stackoverflow.com/questions/71505796}\\
% $E_{14}$ & \url{https://github.com/Azure/MachineLearningNotebooks/issues/1927}\\
% $E_{15}$ & \url{https://stackoverflow.com/questions/64039980}\\
% $E_{16}$ & \url{https://community.wandb.ai/t/vega-code/4605}\\
% \bottomrule
% \end{tabular}
% \label{rq1:post links}
% \end{table}

% \begin{figure}[!t]
%     \centering
%     \begin{minipage}[t]{0.495\textwidth}
%         \includegraphics[width=\textwidth]{figures/rq2/problem_solution_heatmap_macro.pdf}
%         \vspace{-2em}
%         \caption{Normalized mapping between problem inquiries and solution macro-topics based on number of posts.}
%         \label{problem-solution:macro-topic}
%     \end{minipage}
%     \begin{minipage}[t]{0.495\textwidth}
%         \includegraphics[width=\textwidth]{figures/rq2/problem_solution_heatmap.pdf}
%         \vspace{-2em}
%         \caption{A close examination of Environment Management ($\hat{R}_{06}$) in Figure~\ref{problem-solution:macro-topic}.}
%         \label{problem-solution:topic}
%     \end{minipage}
%     \vspace{-1.5em}
% \end{figure}

% \textbf{Stop word selection}: Latent elements, particularly non-topic terms, can distort the perceived distribution of topics in posts. To mitigate this, we curate a list of stop words that are particularly relevant to both software engineering and machine learning contexts. By integrating these tailored stop words into the topic modeling process, we neutralize the impact of such extraneous terms, thereby enhancing the precision of our topic distributions.

% Based on our findings, it is clear that the industry needs to improve tools, methods, and guidelines around asset management. To make things better, we believe that academia and industry should work together and base their efforts on more detailed research. 



% \multirow{19}{*}{\parbox{5cm}{Google \\ search \\ engine}} & MLOps tools & \cite{awan_2022,list_of_top_mlops_tools_2023,dilmegani_2023,oladele_2023} &\\
% \cmidrule{2-4}
% & \parbox{5cm}{machine learning \\ project \\ management tools}  &\cite{Czakon_2023,ashugupta917gfg_2021}&\\
% \cmidrule{2-4}
% & \parbox{5cm}{machine learning \\ experiment \\ management tools}  &\cite{Jenkner_2023,Lewinson_2023,data_science_workflow_2021}&\\
% \cmidrule{2-4}
% & \parbox{5cm}{machine learning \\ lifecycle \\ management tools}  &\cite{ganesh_2023,bellamkonda_2022,Heller_2020}&\\
% \cmidrule{2-4}
% & \parbox{5cm}{machine learning \\ workflow \\ management tools}  &\cite{kaewsanmua_2022}&\\
% \cmidrule{2-4}
% & \parbox{5cm}{machine learning \\ model \\ management tools}  &\cite{Bajaj_2023}&\\
% \cmidrule{2-4}
% & \parbox{5cm}{machine learning \\ data \\ management tools}  &\cite{profisee_2023,dilmegani_2022,weinberg_2021}&\\


% Taking into account all the aforementioned settings, an inquiry is considered ``solved'' only if it is a normal inquiry that has been accepted or closed.

%We then proceed to further refine our post collection for topic modeling by eliminating posts with low-quality titles. Specifically, titles made up solely of numerical values, punctuation marks, escape sequences, non-ASCII characters or tool-related keywords in the Appendix Table~\ref{post title keywords} are excluded. After this filtering process, we end up with $6,754$ Stack Overflow posts, $4,959$ tool-specific posts, and $3,352$ repository-specific posts. Subsequently, we will categorize these inquiries for further analysis. %Using an open card sorting process for aggregation, we can explore patterns that might have been overlooked in a more granular examination of individual topics.

%We also exclude GitHub Discussions and GitLab Issues in this RQ due to the low number of posts, with $43$ and $1$, respectively. 

%For knowledge inquiries, challenges in Code Management are primarily solved by methods in Code Development. Challenges related to Experiment Management are primarily tackled with solutions in Environment Management. For problem inquiries, Environment Management is the predominant solution macro-topic for $62.5\%$ macro-topics. Challenges in Observability Management are commonly addressed with Code Development solutions. 

%We extend an invitation to the broader research community to join in this exploration, aiming to illuminate and address the multifaceted challenges inherent in ML asset management. 

%To ensure the quality and relevance of our dataset, we meticulously review the collected posts, discarding any that do not align with ML asset management.

%We typically use a label format consisting of 2-5 words, beginning with a verb and ending with a noun to meet BERTopic's requirement for context and align with human labeling conventions in the previous literature~\cite{chen2023practitioners}. Adjectives are occasionally included for clarity, while the use of adverbs is minimized. 

% \textbf{Open card sorting}: In open card sorting, every contributor should have an equal say. We want to avoid one contributor's opinion overshadowing others because this can lead to biased labels. Thus, each contributor first labels on its own. Then, they meet to discuss and agree on the labels. The results show a Cohen kappa value of approximately $0.872$, indicating a very high level of agreement.

%We treat tool-specific forums as a collective group because the nature of discussions on these platforms tends to align closely, making them more comparable to each other than to broader platforms such as Stack Overflow or repository-specific forums.

%The following example ($E_{02}$) demonstrates a Stack Overflow problem inquiry about a Python script in Azure DevOps not generating an output CSV in a git folder, despite no errors. 

%The following example ($E_{01}$) demonstrates a Stack Overflow problem inquiry about a Python script in Azure DevOps not generating an output CSV in a git folder, despite no errors. The solution involves using the script's directory as a base and joining it with the relative path of the desired output folder to correctly locate and write output files.

%The following example ($E_{03}$) demonstrates a Stack Overflow problem inquiry in which a user encounters a ``CUDA out of memory'' error while training a BERT model on AWS SageMaker, despite having a small dataset and seemingly ample memory. 

%The following example ($E_{04}$) demonstrates a Stack Overflow problem inquiry about the creation of a feature store in VertexAI with labels. 

%The following example ($E_{05}$) demonstrates a Stack Overflow problem inquiry on how to view a model created through a SageMaker tutorial. 

%The following example ($E_{06}$) demonstrates a problem inquiry from GitHub Issues in which the kedro-kubeflow plugin fails to compile the pipeline when the kedro-mlflow version is set correctly. 

%The following example ($E_{08}$) demonstrates a Stack Overflow problem inquiry about the difficulties in changing the working directory to an AWS S3 bucket from an instance of a SageMaker notebook. 

%The following example ($E_{09}$) demonstrates a Stack Overflow problem inquiry about the undeploying of a model from an endpoint without knowing the model's id. 

%The following example ($E_{11}$) demonstrates a Stack Overflow problem inquiry about an unpickle error when trying to load a trained XGBoost model in Sagemaker. 

%The following example ($E_{13}$) demonstrates a Stack Overflow knowledge inquiry on the progress percentage tracking for a \textit{ParallelRunStep} in a pipeline. 
    
%The following example ($E_{12}$) demonstrates a Stack Overflow knowledge inquiry about sharing an AWS Sagemaker endpoint with a friend to detect credit fraud transactions. 

%The following example ($E_{14}$) demonstrates a Stack Overflow knowledge inquiry on the deployment of the SageMaker pipeline using CDK from a specific URL. 

%The following example ($E_{15}$) demonstrates a Stack Overflow problem inquiry about an error when attempting to share an Azure ML workspace using a Service Principal via the Azure CLI. 

%The following example ($E_{16}$) illustrates a knowledge inquiry about the possibility of viewing the underlying Vega or Vega-lite source code for a visualization panel on the platform `wandb'. 

%The following example ($E_{17}$) demonstrates a Stack Overflow knowledge inquiry on the different runtimes supported by MLRun to execute Python code. 

%The following example ($E_{17}$) demonstrates a Stack Overflow knowledge inquiry on the integration of Hydra and DVC for version control of experiment configuration files without uploading the original configuration files to Git and logging the \textit{git hash} to Hydra by default. 

% [$\hat{C}_{16}$] \textbf{User Interface Management}: 
% \begin{itemize}[leftmargin=1cm]
%     \textbf{Definition}: This macro-topic represents the posts related to design, implementation, and maintenance of visual tools and dashboards that enable users to interact with and interpret machine learning systems, models, and data. It encompasses the creation and management of visual representations of data or information, such as plots ($C_{06}$). User interface management enhances user experience by leveraging visual tools to facilitate effective and intuitive data representation and analysis. \\ 
%     \textbf{Example}: The following example ($E_{16}$) illustrates a knowledge inquiry from Weights\&Biases discussion forum on the accessibility of the underlying source code for a Vega or Vega-lite visualization in a Weights\&Biases panel. \\ 
%     [$E_{16}$] \textit{Is it possible to see the underlying source code of Vega or Vega-lite for a particular panel on wandb?} \\ 
% \end{itemize}

%For $81.25\%$ of the macro-topics, the majority of inquiries come from AzureML\footnote{\url{https://azure.microsoft.com/en-us/products/machine-learning}} or SageMaker\footnote{\url{https://aws.amazon.com/sagemaker}}, underscoring their significance as end-to-end solution platforms. Code Management has the most DVC-related inquiries, indicating possible Git integration problems. Topics related to monitoring and the user interface receive most of their inquiries from Weights\&Biases, pointing to potential difficulties in monitoring and visualization configurations with this tool. 

%However, there is a subtle difference in how these solutions manifest themselves across the two types of inquiry. Knowledge inquiries tend to concentrate more heavily around these macro-topics, indicating that users frequently grapple with the fundamental aspects, such as getting to grips with environment configurations, coding practices, or file operations. Conversely, in problem inquiries, although a substantial number of issues revolve around these critical areas, there is a more varied distribution across other topics. This variation suggests a broader spectrum of complexities, indicating that users, while familiar with the basics, might encounter intricate challenges that go beyond the foundational concepts~\cite{chen2023practitioners}.

%It is essential to consider the proven benefits of asset management in other domains, such as platform engineering, where it has been instrumental in optimizing performance, reducing costs, and managing risks. In the context of machine learning, understanding the perspective of tool users is crucial because they are the primary interactors with these tools. 

% \begin{figure}[!t]
%     \centering
%     \begin{minipage}[b]{0.49\textwidth}
%         \includegraphics[width=\textwidth]{figures/RQ2/Knowledge_solution_heatmap_macro.pdf}
%         \caption{Normalized mapping between  inquiries and solution macro-topics based on number of posts.}
%         \label{knowledge-solution:macro-topic}
%     \end{minipage}
%     \begin{minipage}[b]{0.49\textwidth}
%         \includegraphics[width=\textwidth]{figures/RQ2/Knowledge_solution_heatmap.pdf}
%         \caption{Normalized mapping between knowledge inquiries and solution topics in Environment Management ($\hat{R}_{06}$) based on number of posts.}
%         \label{knowledge-solution:topic}
%     \end{minipage}
% \end{figure}

%As the ML community continues to grow and evolve, addressing these challenges is significant in ensuring efficient and effective development of ML-driven solutions. This feature is especially helpful in software engineering research, since a single concept or function can be articulated using various terminologies. 
%With the prevalence of GPT models in the science domain~\cite{stokel2023chatgpt, owens2023nature, wang2023scientific} (such as medical consulting, code completion, and manuscript editing), we decide to introduce GPT-4 as our content summary assistant. 
%For clarity, these hyperparameters include factors such as the minimum size of a cluster (min\_cluster\_size), the number of outliers generated (min\_samples), and more. 

%Our aim is to understand their similarities and distinctions regarding the challenges associated with ML asset management. Each type of forum, endowed with its unique features, draws ML practitioners from different backgrounds. Stack Overflow caters to a wide spectrum of users, from beginners seeking basic knowledge to professionals seeking advanced troubleshooting guidance~\cite{vasilescu2013stackoverflow,vadlamani2020studying}. In contrast, GitHub Issues is mostly visited by developers aiming to resolve specific issues or suggest new features. Tool-specific forums, meanwhile, act as collecting places for specialized user communities. These forums encourage discussions on customized solutions and best practices, specifically tailored to a particular tool or ecosystem~\cite{squire2015should}. By analyzing the nuances of inquiries posed across these forums, we can identify recurring patterns that can be invaluable to ML practitioners. ML developers can determine which forums are most suitable for their inquiries and for what specific purposes. Tool maintainers can gain insight on how to refine their discussion forums to enhance user experience based on our observations. Additionally, SE researchers can gain valuable insights from the patterns and dynamics of inquiries across these forums. This can highlight clear paths for future research and pinpoint areas that require in-depth investigation.

%In RQ2, we seek to determine which topics are especially challenging to resolve and which require prolonged periods to find resolutions. Understanding the nuances of these challenges is crucial to enhancing user experience. When ML practitioners struggle to find resolutions, not only does this lead to frustration, but it can also stall their progress. By pinpointing these areas of difficulty, SE researchers can be directed towards topics that warrant further investigation. Moreover, by being aware of these challenging topics, application developers can better prepare themselves for potential bottlenecks. For tool developers, such insights are invaluable, providing a clear perspective of market demands and highlighting opportunities for innovation.
 
%\item The tool is a miscategorized tool that lacks asset management core features. The tool is often mislabeled and lacks essential features for asset management. For instance, some GitHub repositories might be tagged as "experiment tracking" but don't primarily offer these capabilities.

%Since it is hard to determine whether a post is in the scope of our study without fully reading the content, we adopt a heuristic strategy to filter irrelevant posts. 

% \textbf{Forum-integrated Learning}: Incorporating forum-integrated learning, particularly in tool-specific forums, can profoundly elevate the learning experience in asset management. Educators have a lot to gain by weaving this interactive medium into their curricula. These forums, renowned for their prompt feedback, serve as effective platforms for students to address classroom-related inquiries, promoting immediate and collective problem solving. By embedding these forums into the academic fabric, students are encouraged to proactively seek solutions, confront real-world challenges, and exchange troubleshooting insights with international peers. Such an engaged learning environment not only promotes collaboration but also sharpens real-time problem solving and critical thinking. Hence, these tool-specific forums not only enrich the learning journey, but also groom professionals geared to adeptly traverse the dynamic realm of asset management.

% However, integration of MLOps practices into the ML development lifecycle introduces numerous challenges, including scalability~\cite{zhou2017machine,chen2020comprehensive}, privacy~\cite{liu2021machine,li2023wind}, standardization~\cite{sculley2015hidden}, and versioning~\cite{zaharia2018accelerating}. These challenges, if they remain unresolved, could impede the effective adoption of ML-driven solutions. One of the most important challenges is machine learning asset management. 

% Machine learning asset management presents unique challenges, especially given the dynamic nature of ML models. These models continuously evolve as they encounter new data, necessitating specialized version control systems. Schelter et al.~\cite{schelter2015challenges} categorize the challenges of managing ML models into three main categories: conceptual, data management, and engineering. in these categories, they highlight the issues of model definition, handling of multiple inputs, metric selection, ensuring data quality, and maintaining compatibility across various programming languages and hardware platforms. 

% This issue is particularly challenging when it comes to machine learning asset management. For instance, the dynamic nature of ML models, characterized by their ability to evolve as they are exposed to new data, requires specialized version control systems. 

% Figure~\ref{fig:github issue-3} shows a problem inquiry\footnote{\url{https://github.com/Lightning-AI/lightning/issues/10397}} from GitHub Issues that is closed due to inactivity. Thus, we define  as the manner by which an inquiry is addressed or concluded, either through a solution, settlement, or other measures. Figure~\ref{fig:github issue-2} shows the resolution found in the comments of a problem inquiry from GitHub Issues.

% In our study, we label inquiries according to the specific situations of resolution. 

% To make terms consistent in different discussion forums, we expand ``no accepted answer rate''\yihao{when you say expand, there has to be an original thing, idk where this ``no accepted answer rate" come from since you didn't explain, or you should say: We name the subset of posts that have no accepted answers as xxx} to ``unresolved rate'' and ``time to accepted answer'' to ``resolution time''. These terms are often used to measure how difficult certain topics are, as referenced in~\cite{bagherzadeh2019going,rosen2016mobile,openja2020analysis,Ahmed2018WhatDC}.

% \begin{figure}
% \includegraphics[width=\columnwidth]{figures/Stack Overflow.png}
% \caption{A resolution from the accepted answer of a problem inquiry in Stack Overflow.}
% \label{fig:stack overflow}
% \end{figure}

% K{\"o}hler~\cite{kohler2022evaluation} provides a detailed evaluation of MLOps tools in a Kubernetes environment, focusing on their functionality, usability, vitality, and performance.

% \yihao{This section needs structured subsections, its now unclear: BG and related work are mixed together; central topic of each background paragraph unclear and would benefit from using sub/subsubsecs, see my commented out summary for each paragarph.}

% \yihao{we need a subsection either here or in introduction (see intro comment) to explicitly, clearly define what is ML asset management and ML (development) lifecycle, with references. So readers know there exists something that is worth knowing before blindly reading the following text.}\ali{agreed. provide examples of ML asset management and lifecycle, and how they relate to eachother. I know you talked about this in intro, but that is not enough.}

% we first provide an overview of the background and foundational concepts related to the ML development lifecycle\yihao{why is it not asset management here, see below for another question on this term}\ali{lifecycle? in intro there was only one place where you used the word lifecycle and i left a long comment on that. Pls fix that and then fix this}\ali{either write something else or explain why you are using the term ``ML development lifecycle'' since it was not being expected by the redaer because in the intro you never hinted that you are headed towards this direction (lifecycle).}.We then discuss previous studies on the management of ML assets. 

% This evolution has consequently catalyzed intertwined developments in the realm of machine learning operations (MLOps). Often likened to DevOps for machine learning, MLOps underscores the symbiotic relationship between data science and IT operations. It ensures that ML models are not only efficiently developed but also adequately maintained, deployed, and monitored. To clarify, while ML asset management focuses on the lifecycle and governance of machine learning assets, MLOps encompasses a broader scope, integrating the entire machine learning lifecycle from development to deployment and monitoring.

%\yihao{Below talks about why ml domain needs MLOps}
% The machine learning domain has undergone a transformative shift in recent decades, evolving from rudimentary algorithms to intricate systems that require sophisticated lifecycles\ali{i dont get this, why would systems need ``sophisticated'' lifecycles?}, operations\ali{of what}, and management frameworks~\cite{kreuzberger2023machine}. This evolution has consequently catalyzed intertwined developments in the realm of ML operationalization (MLOps), which emerged alongside advances in the ML lifecycle\yihao{here, ML development lifecycle vs ML lifecycle vs MLOps I'm confused what is the difference}~\cite{ashmore2021assuring,amershi2019software}\ali{uh! I didnt know what lifecycle is and now we have a new term MLOps that was not used in intro at all}. 

%\yihao{Below talks about MLOps tools+practices are needed beyond traditional DevOps tools+practices}
% \yihao{below seems only talking about ci/cd (at least looks like it), but mlops is more than that, text makes reader think that mlops is just cicd. same problem as in introduction where it only talks about git.}
% Drawing from traditional DevOps practices~\cite{ebert2016devops} that leverage CI/CD for efficient software development, MLOps replicates this efficiency in the ML domain by automating model testing and deployment. Such measures ensure that the models remain relevant and current~\cite{kreuzberger2023machine}. Although previously deploying ML models to production environments could take weeks~\cite{sculley2015hidden}, MLOps tools and practices have expedited this process, allowing organizations to quickly deploy their ML applications. Born from the necessity to seamlessly integrate ML into operational IT environments and built on traditional DevOps principles, but tailored for ML-specific challenges, MLOps marked a pivotal change in ML project management~\cite{kreuzberger2023machine}\yihao{here, another new term - ML project management, btw this sentence feel vague}. The adoption of MLOps not only aims to accelerate the deployment of ML models, but also introduces a positive feedback mechanism for continuous model refinement~\cite{paleyes2022challenges}, \yihao{please add and why is it crucial?}.
% \ali{dedicating a whole paragraph to MLOps idk why.}

%\yihao{Below talks about the challenges practitioners face when adopting MLOps into the ML dev lifecycle and why is it important to address them, with two specific examples: Git and software rollback systems}

% These systems are different from those used in traditional software development, such as Git.
% For instance, the dynamic nature of ML models\ali{why arent you fixing the old concerns jimmy? what is dynamic nature?} requires specialized version control systems that differ from those used in traditional software development, such as Git. Similarly, conventional software versioning systems, such as Git, fall short in the realm of ML due to their inability to address the unique intricacies\yihao{what unique intricacies, you must be specific or remove future phrases like this if you are not sure, this happens a lot of times} of ML model versioning and deployment.
%The rapidly growing collection of MLOps tools highlights the increasing efforts in this area and underscores the need for more empirical evidence to support their adoption.


%\yihao{Below talks about tool-related challenges are prevalent, this looks like the start point of the related work subsection, this should be related_work::PART1 that talks about known challenges.}
% \ali{Here is the first time you mention asset management in this section, but users already forgot what asset management is since you introduced new terms earlier that looks very similar. That is why we need the definition subsection}

% \ali{This starting sentence disconnects readers from previous paragraph. The logic shift is abrupt. Try something like: While advancements in MLOps tools are promising, their full integration into the wider scope of ML asset management presents another set of challenges. [Remove first sentence] Schelter et al. }

% As ML integrates into various sectors\yihao{sector/realm/domain, these three words kept appearing interchangeably, not sure what it means}\ali{sectors of what?}, addressing its tool-related challenges becomes pivotal for the future of ML asset management. 

% \ali{i have the exact same concern as before, i cant get how MLOps, ML asset management, ML asset lifecycle and ML development lifecycle are connected to each other. Perhaps and example with a diagram might help.}

%\yihao{Below talks about effectiveness of current standards to push forward ML asset management, it should be related_work::PART2 about known efforts to address challenges.}
% \yihao{same problem as last one, remove first sentence. Use title to clarify the central topic of this subsubsec, then should be better.}
% Effective management of various ML assets, including models, datasets, and source code, is becoming increasingly important. As a result, there is a growing effort to establish standards throughout the ML development process\ali{so how is this sentence related to your work?}. 

%\yihao{Our study vs previous studies}

% Alshangiti et al.\cite{Alshangiti2019WhyID} investigate challenges in the development of ML applications by studying Stack Overflow posts, revealing the popularity and difficulty of the topic. In a similar vein, Chen et al.\cite{chen2020comprehensive} examine Stack Overflow to understand the problems developers face when deploying deep learning software. 

% While previous studies, such as Idowu et al.~\cite{idowu2021asset}, Schlegel et al.~\cite{schlegel2023management}, and Schelter et al.~\cite{schelter2015challenges} offer a foundational insight into the challenges of ML asset management, our work, derived from the examination of 13,929 Q\&A posts\yihao{until here you first mention the dataset, should be already mentioned in abstract and intro, then here.} from various developer discussion forums, focuses on the perspective of tool users. Leveraging BERTopic models, we extract topics from challenges\yihao{or is it inquries? Please check similar cases throughout this paper} and resolutions based on Q\&A posts, uncovering a comprehensive discussion landscape in asset management\yihao{whereas our key contributions are?}. Unlike previous studies~\cite{Alshangiti2019WhyID, chen2020comprehensive} that only include Stack Overflow as the sole data source\ali{this sentence implies that there are asset management survey on SOF, but is that true?}, we expand our analysis to include other discussion channels such as repository-specific forums (e.g., GitHub Issues) and tool-specific forums (e.g., MLflow Google Group). By analyzing data from various sources, we gain a clearer understanding of the real-world challenges and resolutions in ML asset management.
% \yihao{it almost feels like you are saying previous studies are not finding ``real-world challenges"? I suggest to rephrase, say something like this: This broader approach allows us to capture a more diverse set of user perspectives (also explain what is a user perspective), thereby offering a comprehensive understanding of the challenges and solutions (resolutions?) encountered in real-world ML asset management.}\ali{agreed}

% Machine learning (ML) has a profound impact on industries and daily life by enabling computers to derive useful insights from data and to execute decisions~\ali{what is the benefit? scalability?}\ali{ML executes decisions?}. 
% \ali{the following sentence breaks the reader flow, look at the comment after the following sentence.}
% With the rise of ML, there is an emerging need for ML asset management solutions, as the distinct characteristics of ML introduce challenges that conventional systems struggle to address. 
% \ali{write something linke this: To make ML scalable, impactful, etc. one requires efficient management of ML assets and its processes, however, ML asset management requires specialized tools and solutions because of its differing nature from the conventional software systems.}
% Despite the expansive literature on ML, there remains a gap concerning the direct challenges tool users face, especially in asset management. 
% \ali{write something like this: To address the particularities of ML asset management there are multiple asset management tools available, however, there has not been a comprehensive survey/investigation on what kind of struggles the ML practitioners have to go through in order to manage the ML assets and what kind of issues exist in the already available tools.} In an effort to bridge this gap, our research focuses on the hurdles ML practitioners face with asset management tools and their adopted mitigation strategies\yihao{where does this term come from? theres no mention in paper text}. 
% \ali{fix the prev sentences according to prev suggestions.}
% Diversifying our exploration, we collect insights from a range of developer discussion platforms, extending from Stack Overflow and GitHub/GitLab to specialized tool forums, such as the MLflow Google Group. Through our analysis, we pinpoint 133 specific challenge topics, which we group into 16 macro-topics. Our findings highlight that the most prevalent solutions revolve around software environment and dependency (23.30\%), feature and component development (15.34\%), and file and directory management (9.62\%). Moreover, when applying a 25\% benchmark, we note that 56.25\% (or 9 out of 16) of the macro-topics in knowledge inquiries display a marked self-resolution trend~\ali{I dont get what sef-resolution means}. These insights~\ali{but you didnt mention insights, you stated results} offer valuable guidance for software engineering researchers exploring new research directions~\ali{how?}, tool developers targeting untapped market segments~\ali{how?}, application developers addressing challenges~\ali{such as?}, and MLOps educators designing progressive curricula~\ali{what does this mean?}\yihao{Its uncommon for stackoverflow papers to target implications to educators, check SAIL's previous papers}.
% \end{abstract}\yihao{please add back the specific numbers and methodologies that you deleted from previous version.}

% Our objective is to gain a holistic understanding of user inquiries specific to asset management, marking our paper as a pioneering effort in this perspective\yihao{I would not use pioneering, try something like, to the best of our knowledge, }\ali{re-write this sentence, dont make bold claims the reviewer might be working ont he same idea while reviewing your paper, simplify this thing ``holistic understanding of user inquiries specific to asset management''}.
% These insights \ali{what insights?} are invaluable for software engineering (SE) researchers looking for innovative research avenues\ali{how?}, tool developers identifying emerging markets and features\ali{how?}, application developers aiming to sidestep potential pitfalls\ali{why?}, and MLOps\ali{where did this neww word come from} educators shaping future-focused curricula\ali{why?}.\ali{for this particular sentence, i think i left the same comment on abstract too.}

% Alshangiti et al.\cite{Alshangiti2019WhyID} investigate challenges in the development of ML applications by studying Stack Overflow posts, revealing the popularity and difficulty of the topic. In a similar vein, Chen et al.\cite{chen2020comprehensive} examine Stack Overflow to understand the problems developers face when deploying deep learning software. 


% Although Alshangiti et al.\cite{Alshangiti2019WhyID} and Chen et al.~\cite{chen2020comprehensive} have used Stack Overflow to identify the prevalence and difficulty of these\ali{use a technical word here instead of saying these. do you mean ML asset mgmt? say what you mean here from the word ``these''.} challenges, there remains an untouched area\yihao{what exactly is the untouched area? Let's clarify that asset management domain remains unexplored, \ie we dont know what user  challenges of such tools. I checked both papers and they are not about asset management, they are about development of ML applications?}\ali{what untouched area?}. 
% The existing literature has overlooked\yihao{same as abstract, this word seems aggressive to me idk}\ali{existing literature is limited to .. or dont talk about existing literature ``in this sentence'' at all, that would be the safest apporach.} the direct challenges experienced by ML asset management tools' users, leaving a critical empirical gap~\ali{you are using the word empirical too much. dont use this word more than once in this section. what if there is a paper that did the study same as your and you are not aware of it? Be careful with your words}\yihao{that ... what happens if we dont address the gap, and I thought you already talked about the gap in the previous paragraph.}\ali{agree}. 

% To initiate\ali{do you mean conduct?} our study, we first categorize the inquiries\ali{that are posted by ML practitioners on discussion forums} into problem and knowledge types. 
% We then employ BERTopic~\cite{grootendorst2022bertopic} \ali{(a topic-modelling approach)} to extract the topics of these inquiries. 
% This is followed by an identification of topics that are prevalent in the inquiries and topics that are difficult to find answers for (difficulty analysis). 

% We find that the resolutions most frequently discussed\ali{proposed?} are related to software environment and dependency (23.30\%)\yihao{is this more of expected since a question asking A, then its resolution is expected to be also A right? You could focus on explain the other two different ones than inquiry macro-topic, meanwhile find justifaction for this}, feature and component development (15.34\%), and file and directory (9.62\%). In particular, resolutions tend to align closely with the initial topics of concern. 
% Using a 25\% proportion benchmark\yihao{you said 25\% benchmark in abstract but 25\% proportion benchmark here, but what are they?}, we observe that 56.25\% (9 out of 16) of the challenge macro-topics in knowledge inquiries exhibit a pronounced\yihao{number xyz} self-resolution rate\yihao{not defined, same as abstract}. 
% Conversely, only 25\% (4 out of 16) of the challenge macro-topics in problem inquiries display a similar rate. Diving into the most prevalent resolution macro-topic, software environment and dependency, two main resolution topics stand out. 
% For knowledge inquiries, container customization is the leading resolution, while for problem inquiries, package upgrade is the most common resolution.
% \end{itemize} \yihao{overall, implications are missing.}\ali{at the end of each item in this itemizer, write what are the insights drawn from the stats/results. e.g. result/stat = Ali is 10x fatter than Jimmy. Insight = ML Practitioners should focus more on Ali because he is fatter.}


% \ali{of inquiries? whenever you say topic you have to tell the reader what the topic is of.} linked to challenges\ali{just add a bracket and tell what challenge means}\yihao{we need somewhere in previous text to define what is a ``challenge" and relationship with ``topic".}\ali{correct}, which we subsequently categorize into 16 macro-topics, which are the high-level representations of the challenges~\cite{chen2023practitioners}. 

% An analysis of various tools \ali{this starting breaks the flow of the paragraph. It should either be a new para, or proper start that glues with the previous content.}\ali{btw, you did not analyze tools, so dont say and ``An analysis of various tools''.} reveal inherent challenges\yihao{very vague, what is various tools and why inherent? I dont see these discussions in results section.}\ali{dont use the word challenges unless essential, use it only where you mean actual ``challenge'' that you have defined in your paper.} specific to each. 

%For difficult analysis, we measure the unsolved rate and the resolution time of the inquries to shed light on the difficulties of the challenges \ali{the reader does not know what a challenge means until this point, therefore, they dont know what you mean by shedding light on the difficulties of challenges. Rather, just say that you want to find the topics that are diffuclt to find answers for. KEEP IT SIMPLE}. 

% We expand our research by analyzing insights from developer discussion platforms such as Stack Overflow, GitHub Issues, and tool-specific forums. To our knowledge, this is the first empirical study that systematically investigates user challenges in adopting machine learning asset management tools.
% our objective is to identify the challenges that ML practitioners face when using asset management tools and the strategies they employ to overcome them. 
%Considering both open-source and proprietary ML asset management tools, our study broadens its\yihao{who is it?} scope by incorporating insights from developer discussion platforms, including Stack Overflow, GitHub Issues and tool-specific forums (\ie official forums hosted by the tool maintainers)\ali{take yihao comments into consideration and re-write this sentence}.

% Notably,  stand out as the most prevalent for any designated forum\yihao{``designated forum" not defined yet, its not even defined in RQ3 results.}, even though the frequency distribution of inquiries across macro-topics is consistent across forums\ali{I dont know why stats are missing throughout this paragraph}.

% In contrast, GitHub, which represents 16.87\% of such inquiries\ali{what is ``such'' referring to?}, is the least popular\yihao{is it really popularity or just the nature of the data (Q\&As).}\ali{address this comment in threats}. 
% Generally, GitHub and Stack Overflow inquiries have a longer resolution timeframe \yihao{xyz number} compared to tool-specific forums, which typically offer more rapid \yihao{xyz number} responses.

% Problem inquiries overshadow\yihao{xyz number} knowledge inquiries on these forums and often have a longer resolution time, with an elevated probability of remaining unanswered\ali{stats?}. The forum's nature\yihao{what nature?}\ali{technical nature? unrealistic nature? bad nature? good nature?} influences an inquiry's resolution chances: problem inquiries are harder to resolve on Stack Overflow and tool-specific forums\yihao{This is phenomena not the nature}, while knowledge inquiries face the same challenge on GitHub. 
% The resolution time for both types of inquiry is consistent across different platforms, there are significant differences in the time taken to resolve inquiries for different macro-topics. Nevertheless, the percentage \yihao{xyz number} of unresolved inquiries is consistently uniform across various macro-topics. 



% We find macro-topics related to visualization and user interface, data preparation and preprocessing, as well as model deployment and serving exhibit the highest unresolved rates at 71.43\%, 70.31\%, and 67.63\%, respectively.  In particular, there is a mild\yihao{could that be noise?} negative correlation between resolution time and the unresolved rate of user inquiries across topics.

 % It is worth noting that Specifically, the tool Domino is notably \yihao{do you mean xyz\%} associated with feature and component development inquiries\ali{what does its ``association'' with these two topics imply? cant you simply just say that most of the inquries it has are related to these two topics?}, while the tool Optuna is more related\yihao{are you saying such topics are more challenging in this tool or the tool itself is more related to model creation and training? I cannot understand}\ali{what is the meaning of related?} to model creation and training. 
 
%Usually, a single inquiry can potentially lead to a multitude of resolutions. For example, when faced with a networking related problem, resolution might span the domain of ``network security'', such as addressing a misassigned role, or it might be rooted in proxy configuration, addressing issues such as restoring a stalled internet connection.

%This perspective not only helps in refining the tools but also ensures that they are user-centric, enhancing their adoption and effectiveness in real-world scenarios.

% \begin{figure}[!t]
% \includegraphics[width=\columnwidth]{figures/RQ2/Macro-topics group frequency histogram.pdf}
% \caption{Macro-topics group frequency histogram.}
% \label{rq2:macro-topic group frequency histogram}
% \end{figure}

% Traditional software management tools, such as Git that is used for version control of software, are designed primarily to manage traditional software assets, such as source code and documentation. However, these tools are not natively equipped to track the versions of the underlying ML assets, such as model architectures, hyperparameters, and data splits~\cite{sculley2015hidden}. Naturally, one may wish to employ such already existing tools for the management of ML-based solutions as well.
% However, the unique nature of ML-based solutions poses several challenges that traditional systems are not equipped to handle. 
% For instance, traditional Version Control Systems (VCS) are not specifically designed to efficiently manage large datasets~\cite{sculley2015hidden}, which are an essential part of an ML-based system. 
% Furthermore, traditional VCS 
% Tracking these assets is essential for effective experimentation in an ML-based solution, as it helps validate the consistency between these assets with code and data versions\ali{I dont get this last sentence but I am following along with what you originally wrote. Pls fix it}.
% \yihao{is it only about git (tracking)? This whole paragraph seem to focus on git? What about the other components that are integral to mlops?}\ali{True! why spend a whole para on VCS? :S}

%\ali{This para talks why ML management is different from software management}

% Recent years have seen a surge in the development of asset management tools tailored for ML-based solutions, thanks to collaborative efforts from both academia and industry. From the academic realm, tools such as ModelHub~\cite{miao2017modelhub}, DLHub~\cite{chard2019dlhub}, Pdmdims~\cite{peili2018deep}, Runway~\cite{tsay2018runway}, ModelDB~\cite{vartak2018modeldb}, ModelOps~\cite{hummer2019modelops}, and CANDLE~\cite{wozniak2018candle} serve as prototypes of machine learning experiment management. On the other hand, the industry has contributed with tools such as Polyaxon\footnote{\url{https://polyaxon.com/}}, Kedro\footnote{\url{https://kedro.org/}}, ClearML\footnote{\url{https://clear.ml/docs/latest/docs/}} and cnvrg.io\footnote{\url{https://cnvrg.io/}}, among others. 

% These newly popped tools solve the allevaite a lot about the old issues commonly with traditional software management tools~\cite{sculley2015hidden}.



% Despite the wealth of research on asset management challenges, there remains an empirical gap with respect to challenges from the perspective of tool users\yihao{here we need to state why understanding from the tool users' perspective is crucial, essentially motivates our study}\ali{agreed}. 

% Observability in ML involves understanding the internal state of the system from its external outputs, which allows teams to monitor, diagnose, and troubleshoot issues that may arise during the ML lifecycle~\cite{liu2013observability}.

%Setting our work apart, we cater to the pressing need for empirical research targeting the tangible, on-the-ground challenges tied to asset management, seen from the user's standpoint.

%management of specific assets, such as software environments and ML models, and to explore resolutions tailored to these assets. Additionally, we encourage researchers to study the evolving patterns of ML assets, for example, the commit history of GitHub repositories pertaining to ML projects.

%Our study, which explores the challenges and support related to ML asset management during the ML lifecycle, provides a detailed landscape of current trends and issues. The transition from isolated experimental projects to integrating ML as a core component of organizational workflows highlights the fundamental need to address and understand these challenges. The nature of inquiries on multiple platforms emphasizes the pressing need for more streamlined solutions in the management of ML assets.

% Schelter et al.~\cite{schelter2015challenges} highlight the challenges in ML model management, including model definition, multiple input handling, metric selection, data quality assurance and system compatibility across diverse programming languages and hardware. Additionally, Schlegel et al.~\cite{schlegel2023management} underscore the complexities in maintaining the comparability, traceability, and reproducibility of artifacts throughout the ML development lifecycle. Idowu et al.~\cite{idowu2021asset} highlight that the lack of tool interoperability, standard management practices, and diverse asset types complicate asset management. Although much of the current research focuses on the different aspects of asset management, there is still a noticeable void in empirical studies that address challenges from the perspective of tool users. Alshangiti et al.~\cite{Alshangiti2019WhyID} investigate challenges in the development of ML applications by studying Stack Overflow posts, revealing the popularity and difficulty of the topic. In a similar vein, Chen et al.~\cite{chen2020comprehensive} examine Stack Overflow to understand the problems developers face when deploying DL software. Our research adds a novel dimension to this discourse. We expand our analysis to include other discussion channels such as repository-specific forums (e.g., GitHub Issues) and tool-specific forums (e.g., MLflow Google Group\footnote{\url{https://groups.google.com/g/mlflow-users}}). By analyzing data from various sources, including forums beyond Stack Overflow, we gain a clearer understanding of the real-world challenges and resolutions in ML asset management.

% Our study is motivated to fill the gap by investigating the challenges and support patterns associated with ML asset management by examining the Q\&A inquiries from developer discussion forums, including Stack Overflow, GitHub Issues, MLflow Google Group, and other tool-specific forums. 

%By addressing these complexities, we can bridge knowledge gaps, boost efficiency and productivity, steer the development of pertinent tools and resources, and propel innovation in the realm of machine learning.

% As mentioned in Idowu et al.~\cite{idowu2021asset}, the challenges include , tight coupling with specific libraries, friction, and overhead incurred during usage due to required code instrumentation for tracking assets. They also notes that there is a lack of standardized and explicit management methods to store, version, or operate machine learning assets, and that users rely on ad hoc approaches that may limit their efficiency during model development. Additionally, the varying asset type formats (e.g., different language codebases, models, data, and metrics formats) contribute to this challenge and limit knowledge transfer regarding asset management across various projects. 

%In addition to comparing topics, it is equally important to compare the difficulty of problem inquiries with knowledge inquiries. For example, knowing the relative difficulty of problem and knowledge inquiries can help practitioners prioritize their efforts. If practical problems are identified as more challenging and impactful, then addressing these problems may take precedence over theoretical inquiries, and vice versa. This ensures that the most critical and challenging issues are addressed first, leading to more effective and efficient outcomes.

%Also, we differentiate between ``challenge'' and ``inquiry'' to emphasize that the former represents the overarching issue, while the latter pinpoints the precise question or assistance related to that issue. 
 
%Acknowledging this nuance, we further redefine "solution" as "resolution" when a proposed solution surfaces in the discussion or, sporadically, in the query text itself, a scenario exemplified in Figure~\ref{fig:github issue-2}. 

%For example, a surge in discussions related to the ``dependency constraint'' would emphasize its prevalence and potential significance in the field. Conversely, if questions regarding the ``batch transform'' remain consistently unanswered or elicit unsatisfactory responses, this could suggest inherent complexities or knowledge gaps related to this topic.

 %Sculley et al.\cite{sculley2015hidden} and others\cite{tamburri2020sustainable,symeonidis2022mlops}, has led to the exploration of innovative solutions specific to the versioning and deployment of the ML model. 
%The evolution of the Machine Learning (ML) lifecycle is rooted in the pioneering works of Amershi et al.~\cite{amershi2019software} and Ashmore et al.~\cite{ashmore2021assuring}, which delineate the transformative journey from model requirements to actionable insight. As ML projects have grown in sophistication, so has understanding of this lifecycle, demanding a more methodical approach to its development and maintenance. Modern studies have shed light on the intricate dimensions of each stage, from the criticality of data acquisition to the delicate nuances of model monitoring. The lifecycle of machine learning (ML) is multifaceted, underlining not only the quality and pertinence of the data, but also the challenges associated with data engineering, algorithm selection, model evaluation, real-world deployment, continuous monitoring, and ethical considerations~\cite{polyzotis2018data,arpteg2018software,paleyes2022challenges,giray2021software,chen2020comprehensive}. This complex network of factors, combined with an iterative feedback loop, necessitates a holistic approach that addresses both the technical and socio-ethical dimensions of ML applications. Additionally, it is indispensable for auditing, debugging, and maintaining transparency and accountability throughout the ML development and deployment stages.

%scalability~\cite{sculley2015hidden}. A model that functions well in a limited, controlled setting might struggle when applied to the larger, diverse data of the real world. For example, recommendation systems such as Netflix or Amazon's might excel during testing but encounter issues when handling millions of new daily data inputs, such as user preferences or fresh content. In general, while ML is critical to the advancement of fields from e-commerce to healthcare, the operationalization of ML solutions in production environments presents a myriad of challenges.

%Inquiries focus significantly more on problem solving than on seeking general knowledge on most topics related to machine learning asset management.

%In essence, MLOps democratizes and operationalizes ML, making it an integral and agile part of the organizational workflow rather than an isolated experimental project. Even with the rise of MLOps, managing all the intricacies of an ML project continues to pose challenges~\cite{paleyes2022challenges,giray2021software,ashmore2021assuring,chen2020comprehensive,sculley2015hidden}. %With the multifaceted nature of ML projects, ensuring that results can be replicated consistently in different settings becomes a critical challenge~\cite{hutson2018artificial}. On the one hand, systematic management practices can help keep a detailed record of workflows, configurations, and dependencies, facilitating reproducibility~\cite{chang2022understanding}. On the other hand, the dynamic environment in which machine learning operates, with ever-evolving datasets, algorithms, and hardware, can introduce variations that affect the consistency of results. Therefore, while rigorous documentation is crucial, it is equally important to maintain a controlled environment and be transparent about the inherent uncertainties and variables that might influence reproducibility~\cite{idowu2021asset}.

% \textbf{Problem Inquiries Prevail Discussions}: Since problem inquiries appear more frequently than knowledge inquiries in Q\&A posts, researchers might consider a two-pronged approach: a) design methodologies that prevent these problems from arising, and b) develop effective troubleshooting techniques to address them when they arise.

% \textbf{Focus on Troubleshooting}: Given the prevalence of problem inquiries, educators should put a high emphasis on troubleshooting skills, equipping students with the ability to navigate and resolve issues effectively.

% \textbf{Emphasizing Collaborative Learning}: The findings indicate that ML practitioners frequently turn to forums like Stack Overflow for assistance. Educators can promote collaborative learning, encouraging students to seek and share knowledge in community forums.

% \textbf{Real-world Case Studies}: Educators can integrate real-world case studies and discussions from platforms like GitHub into the classroom, giving students insight into current challenges and resolutions in the ML landscape.

% \textbf{Problem-solving vs. Knowledge-seeking}: Given that problem inquiries prevail discussions, developers must be prepared with robust troubleshooting skills. They should also be proactive in seeking and sharing knowledge, making the community richer in solutions and workarounds.

% \textbf{Enhanced Troubleshooting and Diagnostic Features}: With problem inquiries prevailing the discussions, tool developers should focus on integrating advanced diagnostic and troubleshooting features into their offerings. This could include automated error detection, actionable feedback, solutions to common problems, and links to relevant community discussions or documentation.

% \textbf{Collaborative and Knowledge-sharing Features}: Given the frequent turn to forums for assistance, tool developers could incorporate collaborative features directly into their platforms. Features may include integrated community forums, shared troubleshooting repositories, or even in-tool annotations where users can leave comments, solutions, or best practices for specific functions or issues. This would harness the collective knowledge of the community and make it readily available to all users.

%On the one hand, users on Stack Overflow and tool-specific forums often comprise a diverse set of practitioners, ranging from beginners to experts. Therefore, basic-to-intermediate-knowledge-quest inquiries are likely answered quickly by the community. On the other hand, GitHub discussions are often related to specific software projects, so problem inquiries, like bug reports, can directly affect the project's health. Therefore, maintainers and contributors might be more inclined to address these issues quickly. In all meanstream forums, problem inquiries consistently take longer to be resolved than knowledge inquiries, according to the findings of RQ2.

% We examine whether the difficulty metrics differ at both macro-topic and topic levels. While the Chi-square tests on the unresolved rate reveal no significant difference at either the macro-topic (p-value = 1.0) or topic levels (p-value = 1.0), the Kruskal-Wallis H tests suggest a significant difference in the distribution of resolved times across both levels. Specifically, for macro-topics and topics, the tests return p-values of 0.002 and 0.000, respectively, and corresponding eta-squared values of 0.039 and 0.010, indicating a small effect size. Additionally, we notice that there is some discrepancy between the rank of the unresolved rate and the median resolved time, so we perform Kendall's tau test at both macro-topic and topic levels. For macro-topics, the p-value of 0.041 suggests a slight inverse relationship with a tau value of -0.383. At the topic level, a tau value of -0.169 also reveals a borderline negative association between resolved time and unresolved rate, supported by a significant p-value of 0.004. This implies that, even though certain (macro-)topics have a high rate of unresolved inquiries, once solutions are pinpointed, they are resolved swiftly. This finding is consistent with earlier observations that some topics show contrastive ranks on two measures of difficulty. Given that some topics have quick resolutions once the problem is understood, practitioners might benefit from developing a robust knowledge base or FAQ for these topics. This would help in swiftly addressing similar inquiries in the future.

% Table~\ref{Kendall tau coefficients} shows the Kendall tau coefficients between the resolved time (h) and other collected metrics, such as score count, readability, reading time, link count and line of code, of the collected posts. We find that there is a weak inverse relationship between the score count and the resolved time (h). Similarly, there is a weak inverse relationship between readability and resolved time (h). On the other hand, we find there is a weak positive relationship between resolved time (h) and either reading time (s), link count or line of code.

% \begin{table}[!t]
% \centering
% \caption{Kendall tau coefficients between the resolved time (h) and other collected metrics}
% \begin{tabular}{lll}
% \toprule
% Metrics &    tau &  p-value \\
% \midrule
%  score count & -0.060 &    0.000 \\
%  readability & -0.063 &    0.000 \\
% reading time (second) &  0.070 &    0.000 \\
%   link count &  0.087 &    0.000 \\
%   line of code &  0.065 &    0.000 \\
% \bottomrule
% \end{tabular}
% \label{Kendall tau coefficients}
% \end{table}

%The FDR corrected p-values for each test on these macro-topics are presented in Table~\ref{rq1:p-value of inquiry type in macro-topic}, as suggested by Noble et al.~\cite{noble2009does}.

% To enhance the conclusion validity in open card sorting, it is crucial to manage contributor fatigue. Certain topics or nuances in the material may be hard to grasp. If contributors are presented with an excessive number of posts, they may become tired or overwhelmed, which could influence their classification choices. To counteract this, each contributor is advised to take breaks or stop the session whenever they feel fatigued. Resuming the task only when refreshed can help ensure more consistent and reliable results.

%Using our closed card sorting method, we classify inquiries into two types: knowledge and problem inquiries. , the unresolved rate (\%), and the median resolved time (in hours) 

% Discussions could potentially be influenced by external sources, such as blogs, articles, or tutorials not included in our scraping process. To ensure the accuracy and completeness of our summaries, we meticulously review each post manually, ensuring that vital information is not overlooked inadvertently. 

% Furthermore, the concepts ``resolution'' and ``solution'' are occasionally used interchangeably in the context of Q\&A posts. However, in our study, we draw a distinction between them. Although a resolution can be broader and may involve compromises, decisions, or discussions that lead to a settled state, a solution is typically more concrete and specific than a resolution, focusing on a clear method, answer, or set of steps to address the inquiry.  On the contrary, if the attached comments contain suggestions or measures that contribute to addressing the issue, we regard it as a solution. For example, the concept ``closed'' is specific to repository issue forums. 

% On the one hand, we find that different challenge macro-topics are associated with varying tools. As illustrated in Figure~\ref{tool-challenge:topic}, each block on the heatmap represents the percentage of posts associated with a specific challenge macro-topic for all the curated tools. Notably, \textbf{For $81.25\%$ of the macro-topics (13 out of 16), the majority of inquiries originate from either AzureML (9 out of 16) or SageMaker (4 out of 16).} This highlights their roles as comprehensive end-to-end solution platforms. However, there are exceptions. \textbf{Code Management ($\hat{C}{02}$) sees its highest proportion ($45.10\%$) of DVC inquiries}, implying potential challenges related to its Git integration. Similarly, \textbf{Observability Management ($\hat{C}{13}$) and User Interface Management ($\hat{C}_{16}$) both have the most inquiries from Weights\&Biases, accounting for $24.94\%$ and $64.89\%$ respectively.} This suggests challenges in visualization and monitoring configurations associated with this tool.


% \begin{figure}[!t]
%     \centering
%     \begin{minipage}[b]{0.49\textwidth}
%         \includegraphics[width=\textwidth]{figures/RQ1/Tool_challenge_heatmap_topicwise.pdf}
%         \caption{Mapping between tools and challenge macro-topics based on number of posts (Normalized across all the curated tools).}
%         \label{tool-challenge:topic}
%     \end{minipage}
%     \begin{minipage}[b]{0.49\textwidth}
%         \includegraphics[width=\textwidth]{figures/RQ1/Tool_challenge_heatmap_toolwise.pdf}
%         \caption{Mapping between tools and challenge macro-topics based on number of posts (Normalized across all the challenge macro-topics).}
%         \label{tool-challenge:tool}
%     \end{minipage}
% \end{figure}

%We noted a distinct pattern in the distribution of collected posts, where problem inquiries were more prevalent than knowledge inquiries. To put it in numbers, p

% We present an example of a resolution label for a knowledge inquiry\footnote{\url{https://stackoverflow.com/questions/46359436}} as follows. When a GitHub issue is closed due to lack of activity, it is typically considered resolved, although it may not actually be resolved, and could be tagged as ``na'' if there is no other indication that the issue has been addressed.

% \textit{Inquiry: I am trying to setup [URL] to log my experiment details getting strange error: [CODE] trying in python 2 and python3.}

% \textit{Solution: It seems like comet isn't installed on your machine. You can use: [CODE] take a look at the example projects at: [URL]}

% \textit{Label: install package}

%For example, while GitHub does not have an ``answer acceptance'' indicator, it uses a system to close posts. We look at the open rate or how many posts remain unclosed. Taking into account the different ways forums resolve posts, we have introduced a metric named ``unresolved rate'' to measure challenges in discussion forums. A high unresolved rate might indicate that the questions are complex or need deep insight to answer. When determining the unresolved rate, we omit forums that do not have resolution indicators, such as the status of ``closed'' or ``answer accepted''. The ``resolved time'' metric measures the duration it takes for a post to reach its resolved status. This is computed by assessing the time difference between when the post was created and when it was closed or received its accepted answer.

% \begin{table}
% \centering
% \caption{Difficulty metrics applicable for different discussion forums.}
% \begin{tabular}{p{5em}p{15em}p{15em}}
% \toprule
% Metrics Name & Description & Applicable Discussion forums \\
% \midrule
% open rate & the proportion of posts that remain open. & GitHub, GitLab \\
% unaccepted rate & the proportion of posts that do not have an accepted answer. & Stack Overflow, Amazon SageMaker, Azure Machine Learning, Polyaxon, Vertex AI, Weights \& Biases \\
% median closed time & the median of the time interval between the closed time and creation time of the post. & GitHub, GitLab \\
% median accepted time & the median of the time interval between the creation time of the accepted answer and the post. & Stack Overflow, Amazon SageMaker, Azure Machine Learning, Polyaxon, Vertex AI, Weights \& Biases \\
% \bottomrule
% \end{tabular}
% \label{difficulty metrics}
% \end{table}

% We employ a bootstrapping approach for post-labeling. To begin with, we randomly select 376 posts from the collection using a sample calculator\footnote{https://www.calculator.net/sample-size-calculator.html}. The first and second authors independently perform the initial labeling. Following this, we carry out an inter-rater evaluation to determine whether the current labels are exhaustive and to ascertain whether new labels emerge. If not, we progressively augment the sample size and repeat the labeling process. When the inter-rater assessment indicates substantial agreement, the labeling is carried out independently by the labelers, keeping an eye on the saturation condition. Importantly, to deepen our comprehension of label granularity, we employ GPT-4-32k to preliminarily label the post collection. While these labels are not final, they serve as a valuable reference for manual labeling. This methodology is particularly beneficial as machine learning asset management spans a wide array of domains in ML engineering. Additionally, we find achieving saturation to be a highly challenging task with fewer than 8000 posts. So we eventually complete the labeling of all of the post-collection.

% For problem inquiry, we summarize the symptom by ``adjective + noun'' structure using two to three words only. For those closed posts, we review the comments or accepted answers and detect any mentioned root cause. If the mentioned root cause is different from the problem inquiry symptom, we label it using the ``adjective + noun'' structure with two to three words only. Or else, we assign ``na'' labels. sometimes, the root cause is not mentioned explicitly in the post, but it does not mean the symptoms are the root causes. In this case, we also label it as ``na''. Then we detect if any solution is proposed, and we assign a label for the solution by ``verb + noun'' structure. Note that when there are multiple problem inquiry symptoms, root causes, or solutions detected, we just pick the most commonly sensed (or the answerer believes more important) one for summarization. Sometimes, the root cause or solution is only mentioned in the pull request for GitHub posts. In this case, we check the pull requests instead.

% First, we collect the multivocal literature from multiple sources, such as Google search engine, Github platform, research databases, and industry practitioners. Since ML asset management is a new concept that has recently emerged, we refer to nine stages of the ML workflow outlined in~\cite{amershi2019software} and the five non-exclusive categories of ML support tools~\cite{idowu2021asset} and formulate the following keywords as the search string for multivocal literature retrieval: ``model versioning'', ``model management'', ``model tracking'', ``model development'', ``model serving'', ``model deployment'', ``experiment versioning'', ``experiment management'', ``experiment tracking'', ``pipeline management'' and ``lifecycle management''.

% In general, we refer to three main sources for tool curation: Idowu et al.~\cite{idowu2021asset}, Awesome Production Machine Learning repository\footnote{\url{https://github.com/EthicalML/awesome-production-machine-learning}}, and the Experiment Tracking GitHub topic\footnote{\url{https://github.com/topics/experiment-tracking}}. Idowu et al.~\cite{idowu2021asset} provide a feature-based comparison of 30 tools (18 state of practice and 12 state of research) for ML asset management, highlighting their capabilities in operations, reproducibility, collaboration, and workflow execution. \textit{Awesome Production Machine Learning} is a curated list of open source libraries for the deployment, monitoring, versioning, and scaling of ML applications. The Experiment Tracking topic is a collection of GitHub repositories on the topic related to version control of ML assets during experimentation. 

% There is little consensus as to exactly what MLOps covers. The scope and purpose of MLOps, and thus how it is divided into separate parts, is influenced by the role of the author of the literature addressing it. 

% \subsection{Definition}
% \label{sec:definition}

% \begin{definition}[Machine Learning Life Cycle]
% Machine learning life cycle (MLLC) is a systematic process for planning, building, testing, deploying, and maintaining a machine learning system that ensures the properties, e.g. robustness, fairness, and reproducibility, of the built models.
% \end{definition}

% \begin{definition}[Machine learning pipeline]
% A machine learning pipeline is a means of automating the workflow in machine learning life cycle.
% \end{definition}

% As shown in Figure~\ref{fig:ML Pipeline}, a typical machine learning pipeline consists of three phases: 1) pipeline development, 2) model training, and 3) model serving. The pipeline is usually iterative in its running and is influenced by the model performance based on the business needs.

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Architecture of a machine learning life cycle.png}
% \caption{Architecture of a machine learning life cycle}
% \label{fig:ML Pipeline}
% \end{figure}

% We tentatively define MLOps with the aforementioned concepts below.
% \begin{definition}[MLOps]
% MLOps is a set of practices of machine learning engineering which aims to create a reproducible and continuous pipeline in machine learning life cycle.
% \end{definition}

%\begin{definition}[ModelOps~\footnote{https://www.gartner.com/en/information-technology/glossary/modelops}]
%MLOps is a set of practices of model engineering which aims to create a reproducible and continuous pipeline in artificial intelligence life cycle.
%\end{definition}

% However, ensuring the harmonious integration of all components of the ML system remains a substantial challenge, given the abundance of tools and platforms available for the development and deployment of ML~\cite{kreuzberger2023machine}.
 
%  Addressing these barriers requires a comprehensive approach that considers all aspects of ML asset management, from reproducibility and collaboration to traceability and data privacy. 

%The span of MLOps in ML projects can be as focused or expansive as the project demands as it borrows some of the trusted DevOps best practices such as CI/CD, version control, etc. and adapts them to the new realities of deploying ML models. In certain cases, MLOps can encompass anything from the data pipeline to model production, while other projects may require MLOps implementation of only the model deployment process. 
% As shown in Figure~\ref{fig:Model lifecycle governance}, MLOps is slowly evolving into an independent approach to ML lifecycle governance.
%Though MLOps theoretically covers all aspects of machine learning life cycle, we would like to focus more on the operationalization since it is the core reason the industry introduces the idea of MLOps. 

% \subsection{Technical Concepts}
% \label{sec:backg:concepts}

% This  section  reviews  the  fundamental  terminology  in  MLOps so as to make the study self-contained. 

%Many technologies apply a buzz-word oriented terminology, and occasionally invent their own words to describe what they offer, which may cause some information overload or confusion. 

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Model lifecycle governence.png}
% \caption{Model lifecycle governance}
% \label{fig:Model lifecycle governance}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/MLOps workflow.png}
% \caption{Model lifecycle governance}
% \label{fig:Remove later}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/MLOps blueprint.png}
% \caption{Model lifecycle governance [https://medium.com/slalom-data-analytics/the-modern-mlops-blueprint-c8322af69d21]}
% \label{fig:Remove later}
% \end{figure}

% \subsubsection{Business Understanding}
% Creating a ML model cannot be an end in itself. The model should add value to business, creating new profits or reducing costs. This is where we identify the business problem, collect requirements from the users, and verify how this problem is currently solved, if there is any solution at all. The presented problem can be formulated as one or more machine learning models: classification, regression or others. Also, it is necessary to decide which metrics will be used to evaluate the model. This metric will also allow you to compare the models and determine whether the model is under- or over-fitting. Sometimes, model metrics are always not coherent with the key performance indicator (KPI) in terms of business values. Finally, we should write down all the assumptions and check them. This will allow you to catch errors at an early stage of design.

% Business understanding phase consists of a very precise specification of the business problem together with methods of evaluating the achievement of the goal~\footnote{https://towardsdatascience.com/complete-data-science-project-part-1-business-understanding-b8456bb14bd4}. Our goal is to create a model of the problem, which we use in turn to find a solution. The model should be precise enough to make the solution meaningful, otherwise, we will make too many assumptions and approximations which will make the solution far from real and meaningless. It should be added that real business problems are rarely obvious. Therefore, an iterative approach to the project with multiple repetitions of individual phases is necessary for the solution to be considered acceptable. If we are determined to resort to ML models meet our business needs, we would start to design the data pipeline and move onto the next phase -- Data Preparation.

% \subsubsection{Data(set) Preparation/Transformation}
% In this phase, our main goal is to integrate and enrich the data into an analytical dataset. Usually we first identify the data sources required to build the model. After obtaining the data, we then assess its usefulness based on specific data science standard~\footnote{https://towardsdatascience.com/complete-data-science-project-data-understanding-d4c937a0071c}. For example, we should understand their advantages and limitations, because using poor data model results will also be of low quality~\footnote{GIGO principle: Garbage In Garbage Out}. The data should be representative as well as useful to solve our problem. This process is iterative until the data is ready to ship for the next phase -- Model Development.

% \noindent \textbf{Data sourcing}:  

% \noindent \textbf{Data requirement}:  

% \noindent \textbf{Data understanding}: 

% \noindent \textbf{Data collection}:  

% \noindent \textbf{Data annotation}:  

% \noindent \textbf{Data validation}:  

% \noindent \textbf{Data cleaning}: 

% \noindent \textbf{Data cleansing}: 

% \noindent \textbf{Data lineage}: 

% \noindent \textbf{Data provenance}: 

% \noindent \textbf{Data profiling}: is the process of examining the data available from an existing information source (e.g. a database or a file) and collecting statistics or informative summaries about that data~\ref{Kimball2009TheDW}.

% \noindent \textbf{Data pipeline}: is a series of transformations to data flowing from one end to another.

% \noindent \textbf{Pipeline-as-Code}: is a process of managing and provisioning computing environments in which software systems will be deployed and managed, through the reusable scripts of infrastructure code [3]. It promotes managing the knowledge and experience inside reusable scripts of infrastructure code, instead of traditionally reserving it for the manual-intensive labor of system administrators, which is typically slow, time-consuming, effort-prone, and often even error-prone.

% \noindent \textbf{Data development}: is the process of building a data set for a specific purpose~\footnote{https://www.aihw.gov.au/getmedia/3bdfdd8a-ae98-4ebe-a111-4a3633ebc61f/gdd.pdf.aspx}.

% \noindent \textbf{Exploratory data analysis}: is a technique to analyze data sets to summarize the main characteristics of them using quantitative and visual aspects~\cite{ExploratoryDataAnalysis}.

% \noindent \textbf{Data collecting/acquisition/extraction/collection}: is to collect data from relevant sources before it can be stored, cleaned, preprocessed, and used for further mechanisms.

% \noindent \textbf{Data preprocessing}: is to transform raw data into an understandable format.

% \noindent \textbf{Data streaming}: is data that continuously flows from a source to a destination to be processed and analyzed in near real-time.

% \noindent \textbf{Data labeling/annotation}: is to tag or label data points such as images, text, or audio by a qualified team of people with meaningful information that will be used to train a machine learning model.

% \noindent \textbf{Data curation/ingestion/integration/warehousing}: is to combine data residing in different sources and providing users with a unified view of them~\footnote{http://www.diag.uniroma1.it//~lenzerin/homepagine/talks/TutorialPODS02.pdf}.

% \noindent \textbf{Data discovery}: is the collection and evaluation of data from various sources and is often used to understand trends and patterns in the data.

% \noindent \textbf{CI/CD orchestration}:

% \noindent \textbf{Data standardization}: is the process of converting the structure of disparate datasets into a common data format.

% \noindent \textbf{Data catalog}: is an organized inventory of data assets in the organization~\footnote{https://www.oracle.com/big-data/what-is-a-data-catalog}.

% \noindent \textbf{Data governance}: encapsulates the policies and practices implemented to securely manage the data assets in an organization. is how you ensure data that are used in your business operations, reports, and analysis is accurate, trusted, and can be protected.~\footnote{http://searchdatamanagement.techtarget.com/definition/data-governance}

% \noindent \textbf{Data visualization}: is the graphical representation, e.g. charts, graphs, and maps, of data.

% \noindent \textbf{Data compilation}: is the collation of raw data and their transformation into a format that can be easily manipulated or combined with other data in preparation for further analysis~\footnote{https://inee.org/eie-glossary/data-compilation}.

% \noindent \textbf{Model verification}:

% %\noindent \textbf{Data delivery}:
% \noindent \textbf{Data instance}: is data stored in database at a time slice.

% \noindent \textbf{Data monitoring}: is the act of having procedures, technologies and benchmarks for tracking the quality and usefulness of data~\footnote{https://www.edq.com/glossary/data-monitoring/}.

% \noindent \textbf{Data versioning/version control/tracking}: is the process of creating a unique reference for a collection of data.

% \noindent \textbf{Data transformation}: is the process of converting data from one format into another~\footnote{https://www.cio.com/article/2378615/data-management/agile-comes-to-data-integration.html}.

% \noindent \textbf{Data modeling}: is the process of analyzing and defining all the different data your business collects and produces, and the relationships between those bits of data.

% \noindent \textbf{Data model}: is the artifact of data modeling.

% \noindent \textbf{Data mapping}: is the process of matching fields from one database to another.

% \noindent \textbf{Data review (verification and validation)}: is an act through which the correctness conditions of the data are verified~\footnote{https://www3.epa.gov/ttnamti1/files/ambient/pm25/qa/vol2sec17.pdf}.

% \subsubsection{Model Development/Building (ModelDev)}
% In this phase, our goal is develop the best model to solve the business needs. This process can be further divided into two parts:
% \begin{enumerate}
%     \item Build features to find the best model
%     \item Test the model to make sure it will work
% \end{enumerate} 
% We build, iterate, and test our ML models until we are satisfied with the model performance. In this case, we need to put measures and checks in place across our data pipelines and put model validation parameters in place to make the model deployment more robust and performant. Up next is the Model Deployment phase.

% \noindent \textit{Model prototyping}:

% \noindent \textbf{Model-as-a-Component}:

% \noindent \textbf{Model-as-a-Service}:

% \noindent \textbf{Embedded model}:

% \noindent \textbf{pre-train testing}: is the testing of pre-conditions of training machine learning models, e.g. checking the output ranges and ensuring it aligns with our expectations.

% \noindent \textbf{Model architecture}: defines the various layers involved in the machine learning cycle~\footnote{https://www.educba.com/machine-learning-architecture/}.

% \noindent \textbf{Model creation}: 

% \noindent \textbf{Hyperparameter optimization/tuning}: is the process of searching for a set of hyperparameters that gives the best model results on a given dataset~\cite{Claesen2015HyperparameterSI}.

% \noindent \textbf{Model evaluation}: is the process of quantifying model performance based on the interested metrics.

% %\noindent \textbf{Model generation/building}:
% \noindent \textbf{Model testing/validation}: is the testing of model's ability to generalize, that is, to make correct predictions on new data never seen by the trained model.

% \noindent \textbf{Model visualization}:

% \subsubsection{Model Deployment/Inference}
% In this phase, our goal is to use the model in the real-world applications. This process is the core of MLOps. We would audit our models, e.g. conducting user acceptance testing (UAT), from both a business and IT perspective. If the training-serving skew is unacceptable, we would not approve the model integration and suggest model retraining or even remodeling. Once the models are good enough to serve, they would be profiled and stored in model registry. Then, we deploy the models across multiple environments and ensure them not to disrupt the downstream business applications. Once models are deployed, we would move onto the next phase -- Model Maintenance.

% \noindent \textbf{Model serving}: is to deploy ML model as a web service so that other services can ask for predictions and use the results to make their own decisions~\footnote{https://towardsdatascience.com/tagged/model-serving}.

% \noindent \textbf{User acceptance testing}:

% \noindent \textbf{Model audit/review}:

% \noindent \textbf{Active learning}:

% \noindent \textbf{Model approval}:

% \noindent \textbf{Model validation}:

% \noindent \textbf{Model testing}:

% \noindent \textbf{Model orchestration}:

% \noindent \textbf{Model selection}:

% \noindent \textbf{Model packaging}:

% \noindent \textbf{Model manifestation}:

% \noindent \textbf{Model debugging}:

% \noindent \textbf{Model integration}:

% \noindent \textbf{Model store}:

% \noindent \textbf{Champion-challenger testing}:

% \noindent \textbf{Training-serving skew}:

% \noindent \textbf{Model replacement}:

% \noindent \textbf{Model retraining/tuning/update or remodeling or continuous training}:

% \subsubsection{Model Maintenance}
% In this phase, our main goal is to monitor the effectiveness of the model from a technical (infrastructure, outage, high availability, etc.) and functional (model drift, model performance like AUC, precision, etc.) perspective. Sometimes we might need to fix job errors or even roll back to a stable model version. Once our initial models are operational we need to plan for iterations and continuous delivery of ML models in production. When the performance of the model degrades or the model expires, subsequent selection of the updated models need to be triggered through the continuous integration and continuous delivery (CI/CD) process.

% \noindent \textbf{Data enrichment}: is the process of incorporating new updates and information to the existing dataset to improve accuracy. 

% \noindent \textbf{Model monitoring or continuous monitoring}:

% \noindent \textbf{Model deteriorating}:

% \noindent \textbf{Model migration}:

% \noindent \textbf{Model reuse}:

% \noindent \textbf{Model repurpose}:

% \noindent \textbf{Model update}:

% \noindent \textbf{Model calibration}:

% \noindent \textbf{Model proliferation}:

% \noindent \textbf{Model versioning/version control/tracking/registry}:

% \noindent \textbf{Model diagnostics}:

% \noindent \textbf{Model governance}:

% \noindent \textbf{Model retirement}:

% \noindent \textbf{Model redeployment}:

% \subsubsection{Miscellaneous}
% \noindent \textbf{Role-based access control (RBAC)}: is an approach to restricting network access based on a person's role in an organization~\ref{Ferraiolo2009RoleBasedAC}.

% \noindent \textbf{Continuous testing}:

% \noindent \textbf{Concept drift or model staleness}:

% \noindent \textbf{Data drift}:

% \noindent \textbf{Real/Model drift}:

% \noindent \textbf{Virtual drift}:

% \noindent \textbf{Roll-back}:

% \noindent \textbf{Mathematical drift}:

% \noindent \textbf{Calibration drift}:

% \noindent \textbf{Business drift}:

% \noindent \textbf{Performance drift}:

% \noindent \textbf{Ethical drift}:

% \noindent \textbf{CD4ML}:

% \noindent \textbf{Model stealing}: Another type of adversarial attack is reverse engineering a deployed model by querying its inputs (e.g. via a public prediction API) and monitoring the outputs. The adversarial queries are crafted to maximize the extraction of information about the model in order to train a substitute model. This type of attack is referred to as model stealing.

% \noindent \textbf{Model inversion}: The goal of the adversarial attack is recover parts of the private training set, thereby breaking its confidentialty.

% \noindent \textbf{Data poisoning}: The goal of the adversarial attack is to deliberately corrupt the integrity of the model during the training phase in order to manipulate the produced results. Poisoning attacks are particularly relevant in situations where the machine learning model is continuously updated with new incoming training data.

% \noindent \textbf{Data integrity}:

% \noindent \textbf{Model health}:

% \noindent \textbf{Model decay}:

% \noindent \textbf{Model hosting}:

% \noindent \textbf{Data schema skew}:

% \noindent \textbf{Data value skew}:

% \noindent \textbf{Feature skew}:

% \noindent \textbf{Distribution skew}:

% \section{RQ5 Results}
% \label{sec:rq5-results}

% To answer the first question of RQ3\yihao{rq3?}, we train explainable models over topic prevalence, complexity, and difficulty metrics\yihao{reference/explanation needed for explainable models}. Firstly, we want to find out what factors contribute to challenge openness. Since challenge openness is a binary indicator (True/False), we model it with the gradient boosting decision tree (GBDT) classification model\yihao{reference needed}. To improve the AUC score, we preprocess the training data by applying the feature scaler that is robust to outliers and then imputing the missing values with the k-Nearest Neighbors~\cite{altman1992introduction} technique. Rather than finding the best possible predictor that has the highest possible AUC score, we are more interested in the feature importance in explaining the challenge openness. After a series of bootstrapping hyperparameter searches, our models reach a very high AUC score ($>0.99$) when we set up a high estimator number (1,000) and low max depth number (5). \yihao{these hyperparams all need explanation for what they are and references.}

% % To understand the topic prevalence from a more granular perspective, we conduct rounds of Kruskal-Wallis tests to verify if any prevalence metric is significantly different from the others in terms of macro topics. It shows that platform, tools, challenge topic count, challenge comment count, challenge answer count, and challenge participation count are significantly different from each other ($\alpha$=0.01) across macro topics. 

% Generally, the importance value provides a score that indicates how useful or valuable each feature was in the construction of the boosted decision trees in the GBDT model. The more an attribute is used to make key decisions with decision trees, the higher its relative importance. The importance value is calculated explicitly for each feature in the data, allowing features to be ranked and compared to each other. \yihao{everything before this should be placed into methodologies right?} We find prevalence and complexity metrics differ a bit across GitHub, Stack Overflow, and other platforms, so we model them separately as follows.

% Figure~\ref{fig:Challenge_openness shap_based_feature_importance (GitHub issue)} shows the feature importance to the challenge openness of GitHub issue posts based on SHAP values. It is model-agnostic and uses the Shapley values from game theory to estimate how each feature contributes to the prediction \yihao{same, need reference and explain what do they do}
% % The permutation method randomly shuffles each feature and computes the change in the model’s performance. The features which impact the performance the most are the most important ones. 

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ5/Challenge openness feature importance (Git).png}
% \caption{Feature importance for challenge openness (GitHub issue)}
% \label{fig:Challenge_openness shap_based_feature_importance (GitHub issue)}
% \end{figure}

% Figure~\ref{fig:Challenge_openness shap_based_feature_importance (GitHub issue)} shows features each contributing to push the model output from the base value (the average model output over the training dataset we passed) to the model output. Features pushing the prediction higher are shown in red, those pushing the prediction lower are in blue.

% Figure~\ref{fig:Challenge_openness shap_based_feature_importance (Stack Overflow post)} shows the feature importance to the challenge openness of Stack Overflow posts based on shap values. Note there are demographic metrics available in Stack Overflow posts, so we include them in our model building.

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ5/Challenge openness feature importance (Stack Overflow).png}
% \caption{Feature importance for challenge openness (Stack Overflow post)}
% \label{fig:Challenge_openness shap_based_feature_importance (Stack Overflow post)}
% \end{figure}

% Figure~\ref{fig:Challenge_openness shap_based_feature_importance (Tool-specific post)} shows the feature importance to the challenge openness of tool-specific forum posts based on shap values.

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ5/Challenge openness feature importance (Tool-specific).png}
% \caption{Feature importance for challenge openness (Tool-specific post)}
% \label{fig:Challenge_openness shap_based_feature_importance (Tool-specific post)}
% \end{figure}

% % Secondly, we want to find out what factors contribute to the challenge open time. Since open time (in hours) is a numeric variable ((0, $+\infty$]), we model it with the GBDT regression model. To minimize the MSE (mean squared error), we preprocess the training data using the same steps mentioned earlier. 

% % Figure~\ref{fig:challenge_open_time xgboost_feature_importance (GitHub issue)} shows the feature importance to the challenge open time of GitHub issue posts based on shap values.

% % \begin{figure}[!htb]
% % \centering
% % \includegraphics[width=\columnwidth]{figures/RQ2/Challenge_open_time shap_based_feature_importance (GitHub issue).png}
% % \caption{Feature importance for challenge open time (GitHub issue)}
% % \label{fig:challenge_open_time xgboost_feature_importance (GitHub issue)}
% % \end{figure}

% % Figure~\ref{fig:challenge_open_time xgboost_feature_importance (Stack Overflow post)} shows the feature importance to the challenge open time of Stack Overflow posts based on shap values.

% % \begin{figure}[!htb]
% % \centering
% % \includegraphics[width=\columnwidth]{figures/RQ2/Challenge_open_time shap_based_feature_importance (Stack Overflow post).png}
% % \caption{Feature importance for challenge open time (Stack Overflow post)}
% % \label{fig:challenge_open_time xgboost_feature_importance (Stack Overflow post)}
% % \end{figure}

% % Figure~\ref{fig:challenge_open_time xgboost_feature_importance (Tool-specific post)} shows the feature importance to the challenge open time of tool-specific forum posts based on shap values.

% % \begin{figure}[!htb]
% % \centering
% % \includegraphics[width=\columnwidth]{figures/RQ2/Challenge_open_time shap_based_feature_importance (Tool-specific post).png}
% % \caption{Feature importance for challenge open time (Tool-specific post)}
% % \label{fig:challenge_open_time xgboost_feature_importance (Tool-specific post)}
% % \end{figure}

% Secondly, we want to find out what factors contribute to the challenge solved time. Since solved time (in hours) is also a numeric variable ((0, $+\infty$]), we model it with the GBDT regression model. To minimize the MSE (mean squared error), we preprocess the training data using the same steps mentioned earlier. 

% Figure~\ref{fig:challenge_solved_time xgboost_feature_importance (GitHub issue)} shows the feature importance to the challenge solved time of GitHub issue posts based on shap values.

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ5/Challenge closed time feature importance (Git).png}
% \caption{Feature importance for challenge solved time (GitHub issue)}
% \label{fig:challenge_solved_time xgboost_feature_importance (GitHub issue)}
% \end{figure}

% Figure~\ref{fig:challenge_solved_time xgboost_feature_importance (Stack Overflow post)} shows the feature importance to the challenge solved time of Stack Overflow posts based on shap values.

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ5/Challenge openness feature importance (Stack Overflow).png}
% \caption{Feature importance for challenge solved time (Stack Overflow post)}
% \label{fig:challenge_solved_time xgboost_feature_importance (Stack Overflow post)}
% \end{figure}

% Figure~\ref{fig:challenge_solved_time xgboost_feature_importance (Tool-specific post)} shows the feature importance to the challenge solved time of tool-specific forum posts based on shap values.

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ5/Challenge openness feature importance (Tool-specific).png}
% \caption{Feature importance for challenge solved time (Tool-specific post)}
% \label{fig:challenge_solved_time xgboost_feature_importance (Tool-specific post)}
% \end{figure}

% Lastly, we also explore the factors contributing to the challenge adjusted solved time for Stack Overflow posts. Figure~\ref{fig:challenge_solved_time xgboost_feature_importance (Stack Overflow post)} shows the feature importance to the challenge solved time of tool-specific forum posts based on shap values. We see there are feature importance shifts between challenge solved time and challenge adjusted solved time models.

% % \begin{figure}[!htb]
% % \centering
% % \includegraphics[width=\columnwidth]{figures/RQ2/Challenge_adjusted_solved_time shap_based_feature_importance (Stack Overflow post).png}
% % \caption{Feature importance for challenge adjusted solved time (Stack Overflow post)}
% % \label{fig:Challenge_adjusted_solved_time xgboost_feature_importance (Stack Overflow post)}
% % \end{figure}

% To answer the second question of RQ2, we explore the difficulty and complexity metrics for each macro topic. We conduct rounds of Kruskal-Wallis tests to verify if any difficulty and complexity metric is significantly different from the others in terms of macro topics. It shows that challenge link count, challenge readability, challenge reading time, and challenge sentence count are significantly different from each other ($\alpha$=0.01) across macro topics. Table~\ref{topic difficulty metrics} shows the central tendency of challenge difficulty metrics across different macro topics. %Note the challenge open time indicates how long the challenge has been open.

% \begin{table}[!htb]
% \centering
% \caption{Topic difficulty metrics}
% \begin{tabular}{lrrr}
% \toprule
% Challenge macro topic & Challenge unsolved rate (h) & Challenge median solved time (h) \\
% \midrule
% Computation Management & 73.87 & 51.46 \\
% Data Management & 71.69 & 18.81 \\
% Deployment Management & 67.48 & 27.98 \\
% Lifecycle Management & 67.41 & 21.97 \\
% Model Management & 70.49 & 42.06 \\
% Performance Management & 67.89 & 39.03 \\
% Identity Management & 71.48 & 15.06 \\
% Service Management & 69.66 & 21.88 \\
% \bottomrule
% \end{tabular}
% \centering
% \label{topic difficulty metrics}
% \end{table}

% We hope to find out if there is any correlation between the difficulty metrics, so we conduct a series of Kendall's tau and Spearman correlation rank tests between each pair of difficulty metrics. We find there is indeed a significant correlation between median and mean solved time ($\alpha$=0.01) across challenge topics. %as well as between median and mean open time ($\alpha$=0.01) 

% % \begin{table}[!htb]
% % \centering
% % \caption{Correlation test results between mean and median (adjusted) solved time across original topics}
% % \begin{tabular}{lll}
% % \hline
% % Metrics & Rank test & p-value \\
% % \hline
% % \specialcell{Solved rate\\Median solved time} & Spearman & 0.82 \\
% % \hline
% % \specialcell{Solved rate\\Median solved time} & Kendall’s Tau & 0.88 \\
% % \hline
% % \specialcell{Solved rate\\Mean solved time} & Spearman & 0.35 \\
% % \hline
% % \specialcell{Solved rate\\Mean solved time} & Kendall’s Tau & 0.36 \\
% % \hline
% % \specialcell{Solved rate\\Median adjusted solved time} & Spearman & 0.72 \\
% % \hline
% % \specialcell{Solved rate\\Median adjusted solved time} & Kendall’s Tau & 0.62 \\
% % \hline
% % \specialcell{Solved rate\\Mean adjusted solved time} & Spearman & 0.74 \\
% % \hline
% % \specialcell{Solved rate\\Mean adjusted solved time} & Kendall’s Tau & 0.73\\
% % \hline
% % \specialcell{Mean solved time\\Median solved time} & Spearman & 0.00 \\
% % \hline
% % \specialcell{Mean solved time\\Median solved time} & Kendall’s Tau, & 0.00 \\
% % \hline
% % \specialcell{Mean adjusted solved time\\Median adjusted solved time} & Spearman & 0.05 \\
% % \hline
% % \specialcell{Mean adjusted solved time\\Median adjusted solved time} & Kendall’s Tau & 0.02 \\
% % \hline
% % \end{tabular}
% % \label{correlation test results between mean and median (adjusted) solved time}
% % \end{table}

% Figure~\ref{fig:median vs mean solved time} shows the map between the median and mean solved time across macro topics. 
 
% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ5/Challenge median vs mean solved time.png}
% \caption{Median challenge vs mean solved time}
% \label{fig:median vs mean solved time}
% \end{figure}
% Figure~\ref{fig:median vs mean solved time} shows the map between the median and mean solved time across macro topics. 
 
% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ5/Anomaly unsolved rate vs median solved time.png}
% \caption{Median challenge vs mean solved time}
% \label{fig:median vs mean solved time}
% \end{figure}

% % Figure~\ref{fig:unsolved rate vs median open time} shows the map between the unsolved rate and median open time across macro topics.

% % \begin{figure}[!htb]
% % \centering
% % \includegraphics[width=\columnwidth]{figures/RQ2/Challenge unsolved rate vs median open time.png}
% % \caption{Challenge unsolved rate vs median open time}
% % \label{fig:unsolved rate vs median open time}
% % \end{figure}

% % Figure~\ref{fig:median vs mean open time} shows the map between the median and mean open time across macro topics. 
 
% % \begin{figure}[!htb]
% % \centering
% % \includegraphics[width=\columnwidth]{figures/RQ5/Challenge median vs mean open time.png}
% % \caption{Median challenge vs mean open time}
% % \label{fig:median vs mean open time}
% % \end{figure}

% % Figure~\ref{fig:median solved time vs open time} shows the map between the median solved time and median open time across macro topics.

% % \begin{figure}[!htb]
% % \centering
% % \includegraphics[width=\columnwidth]{figures/RQ5/Challenge median solved time vs open time.png}
% % \caption{Challenge median solved time vs open time}
% % \label{fig:median solved time vs open time}
% % \end{figure}

% Figure~\ref{fig: median solved time (Anomaly)} shows the map between the median and mean solved time across macro topics. 
 
% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ5/Anomaly_solved_time.png}
% \caption{Median solved time for different anomaly macro-topic}
% \label{fig: median solved time (Anomaly)}
% \end{figure}


% \subsubsection{Phase 4: Difficulty modeling}
% \label{sec:method:subsec:design:phase4}

% \textbf{Step~1:} \textit{Feature design for difficulty modeling}

% In this study, our objective was to develop novel characteristics that could influence the likelihood of receiving accepted responses. We have proposed an online tool that forecasts the chances that a question will receive an accepted response. To achieve this, we analyzed a comprehensive set of questions from which we designed several crucial features.

% In an effort to understand the role of question tags, we conducted an in-depth analysis and consequently introduced new features related to post content. These newly introduced features could serve as yardsticks to evaluate the complexity of the post content. However, it is important to note that we intentionally excluded some features such as poster location, as they had the potential to skew our results.

% Table~\ref{metric collection} shows all the metrics collected and postcalculated in our study. There are five types of metrics: ``timestamp'', ``prevalence'', ``complexity'', ``demographics'', and ``difficulty''. ``Timestamp'' metrics refer to the point in time when a specific event takes place. ``Prevalence'' metrics denote the degree of attention a topic receives from professionals. ``Complexity'' metrics represent the intricacy of the textual content. ``Demographics'' metrics provide information about the person who posted the question and those who answered. ``Difficulty'' metrics gauge the level of challenge in solving a specific problem.

% We use two types of metrics to represent the degree of prevalence: ``usage intensity'' and ``support potential''. ``Usage intensity'' mirrors the number of practitioners who can gain from a solution to the issue. The metrics that embody this category encompass the favorite count, view count, and score of the issue post. ``The potential support'' reflects the number of practitioners who are potentially interested in providing support for the challenge. Example metrics include the answer count and comment count of the issue post.

% We also categorize complexity into two specific types of measures in terms of the goal: ``descriptive complexity'' and ``explanatory complexity''. The term ``descriptive complexity'' refers to the level of effort required to clearly articulate the challenge at hand. The indicators of this include the number of hyperlinks, the readability score, and the estimated reading time of the challenge description. On the other hand, ``explanatory complexity'' signifies the amount of effort required to explain the potential solution lucidly. The metrics for this include the word count, its readability score, and the estimated reading time of the answer/comment description. With those metrics ready, we would conduct hyperparameter sweeps for the best prediction models. 

% The table also shows the results of the Shapiro-Wilk test~\cite{shapiro1965analysis} for normality. Note that we use the italics font to represent prevalent metrics that are shown on the webpage, and the bold font to represent difficulty metrics. Some of the metrics are collected from the discussion webpage, such as \texttt{Challenge\_favorite\_count}, while others are calculated post-hoc based on the original text, such as \texttt{Solution\_information\_entropy}. Note that ``descriptive complexity'' metrics like \texttt{Challenge\_word\_count}, \texttt{Challenge\_unique\_word\_count}, \texttt{Challenge\_sentence\_count}, \texttt{Challenge\_information\_entropy}, and \texttt{Challenge\_readability} are commonly used to indicate text complexity in the natural language processing (NLP) domain. Besides, we add \texttt{Challenge\_link\_count} to represent the extra layer of complexity to understanding the full content. 

% \begin{table}[!htb]
% \centering
% \caption{Metrics collection for further analysis}
% \begin{tabular}{llll}
% \hline
% Type & Metric & Description \\
% \hline
% \multirow{3}*{Difficulty} & challenge openness & whether or not the issue post is marked as solved/closed \\
% && challenge solved time & the time (in hours) it takes to close the issue post \\
% && challenge self closeness & whether or not the issue post is closed by the issue poster \\
% \hline
% \multirow{4}*{Timestamp} && challenge created time & the creation time of the issue post \\
% && challenge closed time & the closed time of the issue post \\
% && challenge last edit time & the last edit time of the issue post \\
% && solution last edit time & the last edit time of the accepted answer \\
% \hline
% \multirow{14}*{Prevalence} & \multirow{7}*{Usage Intensity} & challenge score count & the score of the issue post\\
% && repository star count & the number of stars of the repository where the issue post resides \\
% && repository fork count & the number of forks of the repository where the issue post resides \\
% && challenge view count & the number of views of the issue post \\
% && solution score count & the score of the accepted answer \\
% && challenge comment score count & the accumulative score of the comments of the issue post \\
% && solution comment score count & the score of the comments to the accepted answer \\
% & \multirow{7}*{Support Potential} & challenge answer count & the number of answers of the issue post \\
% && challenge comment count & the number of comments of the issue post \\
% && challenge favorite count & the number of favorites of the issue post  \\
% && repository issue count & the number of non-pull-request issues of the repository where the issue post resides \\
% && repository watch count & the number of watches of the repository where the issue post resides \\
% && repository contributor count & the number of contributors of the repository where the issue post resides \\
% && solution comment count & the number of comments to the accepted answer \\ 
% \hline
% \multirow{22}*{Complexity} & \multirow{7}*{Descriptive Complexity} & challenge code count~\cite{yazdaninia2021characterization} & the non-empty line of code (LOC) in the issue post \\ 
% && challenge link count~\cite{yazdaninia2021characterization, wang2018understanding} & the number of web links of the issue post; rather than viewing the count as a whole, we further categorize the links into documentation, example, image, issue, patch, tool, and tutorial \\
% && challenge readability~\cite{kincaid1975derivation} & the approximate representation of the US grade level needed to comprehend the post text \\ 
% && challenge reading time~\cite{demberg2008data} & an approximate syntactic processing time (in seconds) of the post text \\ 
% && challenge word count~\cite{yazdaninia2021characterization, chua2015answers, treude2011programmers, li2012analyzing, yang2011analyzing} & the number of words of the post text \\ 
% && challenge tag count~\cite{yazdaninia2021characterization, calefato2018ask, wang2018understanding, chua2015answers} & the number of tags belonging to the issue post \\
% && challenge topic count & the number of topics belonging to the issue post \\
% & \multirow{15}*{Explanatory Complexity} & challenge comment code count & the non-empty LOC in the comments to the issue post \\ 
% && challenge comment link count & the accumulative number of web links in the comments to the issue post; rather than viewing the count as a whole, we further categorize the links into documentation, example, image, issue, patch, tool, and tutorial \\
% && challenge comment readability & the approximate representation of the US grade level needed to comprehend the comments text to the issue post \\ 
% && challenge comment reading time & an approximate syntactic processing time (in seconds) of the comments text to the issue post \\ 
% && challenge comment word count & the accumulative number of words of the comments text to the issue post \\ 
% && solution code count & the non-empty LOC in the accepted answer \\ 
% && solution link count & the number of web links in the accepted answer; rather than viewing the count as a whole, we further categorize the links into documentation, example, image, issue, patch, tool, and tutorial \\
% && solution readability & the approximate representation of the US grade level needed to comprehend the accepted answer text\\ 
% && solution reading time & an approximate syntactic processing time (in seconds) of the accepted answer text \\ 
% && solution word count & the accumulative number of words of the accepted answer text \\ 
% && solution comment code count & the non-empty LOC in the comments to the accepted answer \\ 
% && solution comment link count & the number of web links in the comments to the accepted answer; rather than viewing the count as a whole, we further categorize the links into documentation, example, image, issue, patch, tool, and tutorial \\
% && solution comment readability & the approximate representation of the US grade level needed to comprehend the comments text to the accepted answer \\ 
% && solution comment reading time & an approximate syntactic processing time (in seconds) of the comments text to the accepted answer \\ 
% && solution comment word count & the accumulative number of words of the comments text to the accepted answer \\ 
% \hline
% \multirow{16}*{Demographics}&\multirow{8}*{Poster}& poster reputation count & the reputation of the issue poster \\
% && poster upvotes & the number of upvotes given to the issue poster \\
% && poster downvotes & the number of downvotes given to the issue poster \\
% && poster view count & the number of views given to the issue poster \\
% && poster aws employment & whether or not the issue poster is an AWS employee \\
% && poster cloud security engineer certificate & whether or not the issue poster is a cloud security engineer \\
% && poster expertise & whether or not the issue poster is a subject matter expert \\
% && poster moderator role & whether or not the issue poster is a content moderator \\
% &\multirow{8}*{Answerer}& answerer reputation count & the reputation of the accepted answer poster \\
% && answerer upvotes & the number of upvotes given to the accepted answer poster \\
% && answerer downvotes & the number of downvotes given to the accepted answer poster \\
% && answerer view count & the number of views given to the accepted answer poster \\
% && answerer aws employment & whether or not the accepted answer poster is an AWS employee \\
% && answerer cloud security engineer certificate & whether or not the accepted answer poster is a cloud security engineer \\
% && answerer expertise & whether or not the issue poster is a subject matter expert \\
% && answerer moderator role & whether or not the accepted answer poster is a content moderator \\
% \hline
% \multirow{2}*{Miscellaneous} && platform & the platform where the issue post resides \\
% && tools & the toolset where the issue post refers to \\
% \hline
% \end{tabular}
% \label{metric collection}
% \end{table}

% \textbf{Step~2:} \textit{Hyperparameter sweep for difficulty modeling}

% To evaluate our proposed features with respect to getting
% accepted responses, we conduct rounds of grid search over the hyperparameter space of a binary xgboost classifier~\cite{chen2016xgboost}. To ensure the legitimacy of our developed models, we employed a five-fold cross-validation technique. This approach is effective in preventing the occurrence of overfitting~\cite{}. 

% We gauged the efficacy of our classifiers utilizing the AUC or Area Under the Curve, which is a metric commonly associated with the Receiver Operating Characteristic. The AUC value ranges between 0 and 1. A purely random classifier would yield an AUC value of 0.5. The classifiers become more informative as the AUC values increase, and a flawless classifier would achieve an AUC value of 1. Contrary to measures that depend on a certain threshold such as sensitivity and the F-score~\cite{}, the AUC proves to be preferable as it does not depend on a specific classification threshold. It also weighs both the costs and benefits and is suggested as a comparative measure for classifiers~\cite{}. Having the model with the highest AUC score, we then compare the learning curve lest the model overfits the training data. 

% Then we evaluate our proposed features with respect to the time getting accepted answers by grid search over the hyperparameter space of the xgboost regressor. We gauged the efficacy of our classifiers utilizing the RMSE, which represents the quadratic mean of predicted values and observed values of the second sample moment. The other setup is the same as the binary classifier above. Drawing from the above-mentioned methodology, we are able to pinpoint crucial features that could significantly impact the likelihood of answers being accepted and how much time it takes to solve.

%Besides the tools mentioned in~\cite{idowu2021asset}, we also resort to the well-known ML community, \ie~\textit{Awesome Production Machine Learning}~\footnote{github.com/EthicalML/awesome-production-machine-learning} to include more tools. Particularly, we look into the module:~\textit{Commercial Platforms} and~\textit{Model Serving and Monitoring}. We read the official documentation for each tool and check if it ever contains statements regarding~\textit{experiment tracking} or~\textit{version control}. We also check the maintenance conditions of the repository if the tool is open-source. Notably, we exclude~\textit{Datmo},~\textit{Feature Forge},~\textit{StudioML},~\textit{Sumatra}, and~\textit{Deepkit} because all of them kept inactively or no longer maintained (> 1 year period in both last release/commit/PR, open issues, etc.) and drew little attention from the community (few \#star, \#fork, \#watch, \#PR, \#issue, \#branch, \#contributor, etc.) for the last few years. We also exclude~\textit{Dot Science} since the company had shut down, and the tool became inaccessible to us. 

%These professionals often wrestle with a variety of problems, highlighting the need to understand the specific challenges they face in their day-to-day operations\ali{this sentence is too abstract and does not fit to the topic}. 


% \yihao{You need to write some explanation here otherwise I dont see why we need a list of hypothesis in the first place? - they also need to be addressed in the results section.}
% Hypothesis 1: Specific topics are more prevalent than others in terms of post count.
% Hypothesis 2: The topic distribution measured in view count vary from post count.
% Hypothesis 3: The topic distribution measured in score count vary from post count.
% Hypothesis 4: Specific topics are more prevalent than others in terms of answer count.
% Hypothesis 5: The topic distribution measured in comment count vary from answer count.
% Hypothesis 6: The topic distribution measured in participation count vary from answer count.

% Due to the generality overarching of RQ1, a deeper exploration into the specifics of the post-collection process~\ali{what is post collection process, it wasnt explained in the text before this statement} is warranted\yihao{maybe cite something}. For this~\ali{replace `this' with something that connects with the previous sentence}, we individually~\ali{do you mean manually?} examined each post, classifying it into one of three categories: ``knowledge inquiry'', ``problem inquiry''~\ali{make sure this is a famous SE term}, or ``not applicable'' (NA).

% Often, an problem inquiry can exhibit symptoms that are not related to the core problem causing it. In such scenarios, it is crucial to uncover the core issue, referred to as the "root cause". This is vital if the root cause is not evidently linked to the problem inquiry.%example

% When multiple root causes are not visibly connected to the problem inquiry symptoms, it indirectly points toward the concealed technical debts discussed in Sculley's paper~\cite{sculley2015hidden}\ali{this is hard to parse, please explain with an example}. Visualizing a challenge-solution flow through a heatmap can help practitioners to recognize the most common root cause in their routine operations\ali{i think you want to say that a mapping between root cause and its solution is useful, instead of using a technical word of heatmap}. This awareness\ali{mapping} could reduce problem solving time and provide insight into potential avenues\ali{potential avenues? This is verbose and the text can be reduced to the point} for improving asset management tools.

% However\ali{what are we howevering, there needs to be a backing to the word however}, identifying the root cause can be complex due to its hidden nature\ali{what is the meaning of hidden nature, example or expalnation required}. Our method of determining it\ali{what is `it' refering to?} relies solely on resolved cases. Occasionally\ali{does that happen occasionally}, if a case lacks any hint of the root cause, we automatically consider the observable symptom\ali{what is the meaning of observable symptom, explain or provide example} as the root cause.



% In our analysis of common challenges identified in technical issue discussion forums, including both issues and discussion posts, we have determined that every topic can be distinguished by three distinct attributes: prevalence, complexity, demographics, and difficulty. Prevalence is a measure of how much attention a challenge attracts; complexity is a measure of the effort required to comprehend the issue, demographics is the meta-information about the crucial participants such as poster and answerer; and difficulty is a measure of the resources required to resolve the challenge. Table~\ref{metric collection} illustrates each kind of attribute, its constituents, and the corresponding descriptions. Particularly, we are interested in the comparison of difficulty metrics among post topics.


% \textbf{RQ$_6$:} \textit{What factors contribute to the difficulty of the challenge?}

% Our primary interest lies in understanding how other metrics (demographics, prevalence, complexity) impact the difficulty metrics. As such, we have focused our study on exploring these relationships, with an emphasis on creating accurate and explainable prediction models. %Therefore, we have broken down the primary objective of our study into the following three research questions:

% Developers frequently utilize discussion forums or issue discussion channels to address their challenges, functioning either as visitors seeking solutions or as askers posing questions. For example, Stack Overflow serves as a reservoir of validated information, with users particularly interested in accepted answers due to their proven reliability. However, there is an escalating trend of unresolved queries in the community. Therefore, our study aims to determine how accurately we can predict whether a question will garner an accepted answer based on its distinctive characteristics.

% Our study focuses primarily on two parameters: challenge openness and challenge solved time. The term 'challenge openness' indicates the degree of difficulty involved in resolving a suggested issue. On the other hand, 'challenge solved time' signifies the amount of effort required to successfully close an issue. This investigation is significant because it can offer insights into factors that increase the probability of receiving an accepted answer, ultimately helping to resolve more questions. In addition, this research attempts to identify the most crucial features that predict whether a question will be met with an accepted response. Our findings can aid in enhancing the platform's functionality and its ability to facilitate knowledge exchange among developers.

%We measure the difficulty of a challenge in terms of different metrics including the unsolved rate and median closed time. Some types of challenges can be quite prevalent in practical settings and, yet, less difficult than others. In cases like this, raising awareness of simple solutions to these challenges can facilitate the work of ML practitioners in a quick manner. On the other hand, certain types of challenges can be rarer but much more difficult to cope with. An example could be data labeling. Such questions are rarely asked but it is among the most difficult topics to get an answer. Cases like this could point to opportunities for future work in such a way that researchers could further explore mechanisms to cope with that particular problem in an easier and less costly way. Particularly, if a topic is both prevalent and difficult, the topic should receive much more attention from the communities. 

%RQ2 also wants to explore the factors that contribute to the difficulty of a challenge. For each difficulty metric, we train respective supervised learning models for major communities \yihao{e.g. sagemaker?}. By comparing the contribution factors (e.g. feature importance), we determine the degree of usefulness of a specific metric for the difficulty model.

%Thus, quantitatively measuring the difficulty level of questions is important to drive ML development teams in allocating resources to critical operations in the ML production domain both effectively (\ie in a way that the problem is fixed properly) and efficiently (\ie with reduced time to perform the fixes). Through RQ3, we aim at computing the difficulty level of the types of questions identified through the topic extraction performed in RQ1 by computing statistics metrics such as ``no accepted answer ratio'' and ``median hours to accepted answer''. 

% On the one hand, some asset management challenges can be pretty frequent in industry settings and, yet, less difficult than others. Raising awareness of simple solutions to these challenges can quickly facilitate ML practitioners' daily work. On the other hand, some questions are rarely asked, but it is among the most challenging topics to get an answer to. Cases like this could point to opportunities for future work so that researchers could further explore mechanisms to cope with that particular challenge in an easier and less costly way. Thus, quantitatively measuring the difficulty level of challenges is essential to drive ML production teams in allocating resources to critical operations effectively (\ie in a manner that the challenges are fixed properly) and efficiently (\ie with reduced time to perform these fixes).

%ML practitioners are under tremendous pressure to keep up with the new technologies~\cite{Wilson2004PerceptionsOS}. Thus, we use Stack Overflow as a source of information for topics that people should pay more attention to, e.g. by improving current tools to support them in practical settings. We want to understand the difficulty evolution over time and the correlation between the difficulty level and prevalence of the types of challenges. %Lastly, we compare commonalities and variabilities of difficulty metrics across communities, tools, and openness. This is the first quantitative analysis to systematically analyze the difficulty of asset management-related challenges.

% Hypothesis 1: ``Complexity'' metrics contribute positively to a challenge difficulty.
% Hypothesis 2: ``Prevalence'' metrics contribute negatively to a challenge difficulty.
% Hypothesis 3: ``Demographics'' metrics also contribute to a challenge difficulty.
% Hypothesis 4: Specific topics are more difficult than others in terms of unsolved rate.
% Hypothesis 5: Specific topics are more difficult than others in terms of median solved time.

%\textbf{RQ$_3$:} \textit{How does the difficulty of these challenges evolve? How do the factors contributing to the challenge difficulty evolve faced by ML practitioners regarding asset management?} \yihao{update: Consider remove this RQ as it is shaky (meeting discussed)}

%Besides knowing the landscape of prevalence and difficulty metrics in the whole history, we aim at assessing how these types of challenges evolve to identify trends in the past few years. Also, we explore the evolutionary trends of feature importance of the difficulty models. Thus, we have a more dynamic view of why the difficulty metrics have evolved so far. Overall, RQ3 can provide clues to foresee the future prospect regarding the ML asset management discipline.

%Hypothesis 1: Most topics are becoming more prevalent recent years.
%Hypothesis 2: Most topics are becoming more complex recent years.
%Hypothesis 3: Most topics are becoming less difficult recent years.
%Hypothesis 4: ``Complexity'' metrics are contributing less to a challenge difficulty recent years.
%Hypothesis 5: ``Prevalence'' metrics are contributing more to a challenge difficulty recent years.


% In RQ3, we explore the evolutionary trend of difficulty metrics as well as the contributive factors. Firstly, we visualize the difficulty metrics across macro topics with time using LOWESS smoothing regression~\cite{cleveland1979robust}. 

% Figure~\ref{fig:Challenge_unsolved_rate evolution} shows the evolution of the challenge unsolved rate across macro topics. 

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_unsolved_rate.png}
% \caption{Challenge unsolved rate evolution}
% \label{fig:Challenge_unsolved_rate evolution}
% \end{figure}

% Figure~\ref{fig:Challenge_median_open_time evolution} shows the evolution of the median challenge open time (i.e. how long does a challenge keep open?) across macro topics. Note that we do not draw the evolution of challenge adjusted solved time since the only difference between challenge solved time and challenge adjusted solved time arises from the data in Stack Overflow, which leads to a similar pattern to the evolution of challenge solved time overall.

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_open_time.png}
% \caption{median challenge open time evolution (log scale)}
% \label{fig:Challenge_median_open_time evolution}
% \end{figure}

% Lastly, we visualize the evolution of the feature importance contributing to the modeling of difficulty. 

% Figure~\ref{fig:Challenge_openness feature importance evolution (GitHub issue)} shows the evolution of the feature importance of challenge openness for GitHub issue posts across macro topics.

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_openness feature importance evolution (GitHub issue).png}
% \caption{Challenge openness feature importance evolution (GitHub issue)}
% \label{fig:Challenge_openness feature importance evolution (GitHub issue)}
% \end{figure}

% Figure~\ref{fig:Challenge_openness feature importance evolution (Tool-specific post)} shows the evolution of the feature importance of challenge openness for tool-specific forum posts across macro topics.

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_openness feature importance evolution (Tool-specific post).png}
% \caption{Challenge openness feature importance evolution (Tool-specific post)}
% \label{fig:Challenge_openness feature importance evolution (Tool-specific post)}
% \end{figure}

% Figure~\ref{fig:Challenge_openness feature importance evolution (Stack Overflow post)} shows the evolution of the feature importance of challenge openness for Stack Overflow posts across macro topics.

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_openness feature importance evolution (Stack Overflow post).png}
% \caption{Challenge openness feature importance evolution (Stack Overflow post)}
% \label{fig:Challenge_openness feature importance evolution (Stack Overflow post)}
% \end{figure}

% % Figure~\ref{fig:challenge_open_time xgboost_feature_importance (GitHub issue)} shows the evolution of the feature importance of challenge open time for GitHub issue posts across macro topics.

% % \begin{figure}[!htb]
% % \centering
% % \includegraphics[width=\columnwidth]{figures/RQ3/challenge_open_time feature importance evolution (GitHub issue).png}
% % \caption{Challenge open time feature importance evolution (GitHub issue)}
% % \label{fig:challenge_open_time feature importance evolution (GitHub issue)}
% % \end{figure}

% % Figure~\ref{fig:challenge_open_time feature importance evolution (Tool-specific post)} shows the evolution of the feature importance of challenge open time for tool-specific forum posts across macro topics.

% % \begin{figure}[!htb]
% % \centering
% % \includegraphics[width=\columnwidth]{figures/RQ3/challenge_open_time feature importance evolution (Tool-specific post).png}
% % \caption{Challenge open time feature importance evolution (Tool-specific post)}
% % \label{fig:challenge_open_time feature importance evolution (Tool-specific post)}
% % \end{figure}

% % Figure~\ref{fig:challenge_open_time feature importance evolution (Stack Overflow post)} shows the evolution of the feature importance of challenge open time for Stack Overflow posts across macro topics.

% % \begin{figure}[!htb]
% % \centering
% % \includegraphics[width=\columnwidth]{figures/RQ3/challenge_open_time feature importance evolution (Stack Overflow post).png}
% % \caption{Challenge open time feature importance evolution (Stack Overflow post)}
% % \label{fig:challenge_open_time feature importance evolution (Stack Overflow post)}
% % \end{figure}

% Figure~\ref{fig:challenge_solved_time xgboost_feature_importance (GitHub issue)} shows the evolution of the feature importance of challenge solved time for GitHub issue posts across macro topics.

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/challenge_solved_time feature importance evolution (GitHub issue).png}
% \caption{Challenge solved time feature importance evolution (GitHub issue)}
% \label{fig:challenge_solved_time feature importance evolution (GitHub issue)}
% \end{figure}

% Figure~\ref{fig:challenge_solved_time feature importance evolution (Tool-specific post)} shows the evolution of the feature importance of challenge solved time for tool-specific forum posts across macro topics.

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/challenge_solved_time feature importance evolution (Tool-specific post).png}
% \caption{Challenge solved time feature importance evolution (Tool-specific post)}
% \label{fig:challenge_solved_time feature importance evolution (Tool-specific post)}
% \end{figure}

% Figure~\ref{fig:challenge_solved_time feature importance evolution (Stack Overflow post)} shows the evolution of the feature importance of challenge solved time for Stack Overflow posts across macro topics.

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/challenge_solved_time feature importance evolution (Stack Overflow post).png}
% \caption{Challenge solved time feature importance evolution (Stack Overflow post)}
% \label{fig:challenge_solved_time feature importance evolution (Stack Overflow post)}
% \end{figure}

% Figure~\ref{fig:challenge_adjusted_solved_time feature importance evolution (Stack Overflow post)} shows the evolution of the feature importance of challenge adjusted solved time for Stack Overflow posts across macro topics.

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/challenge_adjusted_solved_time feature importance evolution (Stack Overflow post).png}
% \caption{Challenge adjusted solved time feature importance evolution (Stack Overflow post)}
% \label{fig:challenge_adjusted_solved_time feature importance evolution (Stack Overflow post)}
% \end{figure}

% Then we visualize the complexity metrics across macro topics with time. Figure~\ref{fig:Challenge_word_count evolution} shows the mean word count with time across macro topics. 

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_word_count.png}
% \caption{Challenge word count evolution}
% \label{fig:Challenge_word_count evolution}
% \end{figure}

% Figure~\ref{fig:Challenge_sentence_count evolution} shows the mean sentence count with time across macro topics. 

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_sentence_count.png}
% \caption{Challenge sentence count evolution}
% \label{fig:Challenge_sentence_count evolution}
% \end{figure}

% Figure~\ref{fig:Challenge_link_count evolution} shows the mean link count with time across macro topics. 

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_link_count.png}
% \caption{Challenge link count evolution}
% \label{fig:Challenge_link_count evolution}
% \end{figure}

% Figure~\ref{fig:Challenge_readability evolution} shows the mean readability with time across macro topics. 

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_readability.png}
% \caption{Challenge readability evolution}
% \label{fig:Challenge_readability evolution}
% \end{figure}

% Figure~\ref{fig:Challenge_reading_time evolution} shows the mean unique word count with time across macro topics. 

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_reading_time.png}
% \caption{Challenge reading time evolution}
% \label{fig:Challenge_reading_time evolution}
% \end{figure}

% Then, we visualize the evolution trends of the prevalence metrics curve across macro topics. Since all prevalence metrics have increased over the past few years, it is better to compare their increase rate rather than their absolute count.

% Figure~\ref{fig:Challenge_topic_count_increase_rate evolution} shows the evolution of the increase rate of challenge topic count across all macro topics.

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_topic_count_increase_rate.png}
% \caption{Challenge topic count increase rate}
% \label{fig:Challenge_topic_count_increase_rate evolution}
% \end{figure}

% Figure~\ref{fig:Challenge_favorite_count_increase_rate evolution} shows the evolution of the increase rate of challenge favorite count across all macro topics. 

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_favorite_count_increase_rate.png}
% \caption{Challenge favorite count increase rate}
% \label{fig:Challenge_favorite_count_increase_rate evolution}
% \end{figure}

% Figure~\ref{fig:Challenge_score_count_increase_rate evolution} shows the evolution of the increase rate of challenge score across all macro topics.

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_score_count_increase_rate.png}
% \caption{Challenge score count increase rate}
% \label{fig:Challenge_score_count_increase_rate evolution}
% \end{figure} 

% Figure~\ref{fig:Challenge_view_count_increase_rate evolution} shows the evolution of the increase rate of challenge view count across all macro topics. 

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_view_count_increase_rate.png}
% \caption{Challenge view count increase rate}
% \label{fig:Challenge_view_count_increase_rate evolution}
% \end{figure}

% Figure~\ref{fig:Challenge_answer_count_increase_rate evolution} shows the evolution of the increase rate of challenge answer count across all macro topics. 

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_answer_count_increase_rate.png}
% \caption{Challenge answer count increase rate}
% \label{fig:Challenge_answer_count_increase_rate evolution}
% \end{figure}

% Figure~\ref{fig:Challenge_comment_count_increase_rate evolution} shows the evolution of the increase rate of challenge comment count across all macro topics. 

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_comment_count_increase_rate.png}
% \caption{Challenge comment count increase rate}
% \label{fig:Challenge_comment_count_increase_rate evolution}
% \end{figure}

% Figure~\ref{fig:Challenge_participation_count_increase_rate evolution} shows the evolution of the increase rate of challenge participation count across all macro topics. 

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_participation_count_increase_rate.png}
% \caption{Challenge participation count increase rate}
% \label{fig:Challenge_participation_count_increase_rate evolution}
% \end{figure}

% Figure~\ref{fig:Challenge_closed_topic_count_increase_rate evolution} shows the evolution of the increase rate of challenge topic closed count across all macro topics.

% \begin{figure}[!htb]
% \centering
% \includegraphics[width=\columnwidth]{figures/RQ3/Challenge_topic_closed_count_increase_rate.png}
% \caption{Challenge topic closed count increase rate}
% \label{fig:Challenge_closed_topic_count_increase_rate evolution}
% \end{figure}

% Firstly, we visualize the topic count evolution trend (using LOWESS) and three-sigma confidence bound ($\alpha$=0.003) for each macro topic on a monthly frequency. Figure~\ref{fig:Challenge_topic_count (Code Management)} shows the evolution of challenge topic count in \texttt{Code Management}. Figure~\ref{fig:Challenge_topic_count (Data Management)} shows the evolution of challenge topic count in \texttt{Data Management}. Figure~\ref{fig:Challenge_topic_count (Model Management)} shows the evolution of challenge topic count in \texttt{Model Management}. Figure~\ref{fig:Challenge_topic_count (Lifecycle Management)} shows the evolution of challenge topic count in \texttt{Lifecycle Management}. Figure~\ref{fig:Challenge_topic_count (Infrastructure Management)} shows the evolution of challenge topic count in \texttt{Infrastructure Management}. Figure~\ref{fig:Challenge_topic_count (Deployment Management)} shows the evolution of challenge topic count in \texttt{Deployment Management}. Figure~\ref{fig:Challenge_topic_count (Report Management)} shows the evolution of challenge topic count in \texttt{Report Management}. Figure~\ref{fig:Challenge_topic_count (Security Management)} shows the evolution of challenge topic count in \texttt{Security Management}. TODO:


% Secondly, we visualize the view count evolution trend (using LOWESS) and three-sigma confidence bound ($\alpha$=0.003) for each macro topic on a monthly frequency. Figure~\ref{fig:Challenge_view_count (Code Management)} shows the evolution of challenge view count in \texttt{Code Management}. Figure~\ref{fig:Challenge_view_count (Data Management)} shows the evolution of challenge view count in \texttt{Data Management}. Figure~\ref{fig:Challenge_view_count (Model Management)} shows the evolution of challenge view count in \texttt{Model Management}. Figure~\ref{fig:Challenge_view_count (Lifecycle Management)} shows the evolution of challenge view count in \texttt{Lifecycle Management}. Figure~\ref{fig:Challenge_view_count (Infrastructure Management)} shows the evolution of challenge view count in \texttt{Infrastructure Management}. Figure~\ref{fig:Challenge_view_count (Deployment Management)} shows the evolution of challenge view count in \texttt{Deployment Management}. Figure~\ref{fig:Challenge_view_count (Report Management)} shows the evolution of challenge view count in \texttt{Report Management}. Figure~\ref{fig:Challenge_view_count (Security Management)} shows the evolution of challenge view count in \texttt{Security Management}. TODO: 

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_view_count_Code Management.png}
% \caption{Challenge view count (Code Management)}
% \label{fig:Challenge_view_count (Code Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_view_count_Data Management.png}
% \caption{Challenge view count (Data Management)}
% \label{fig:Challenge_view_count (Data Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_view_count_Model Management.png}
% \caption{Challenge view count (Model Management)}
% \label{fig:Challenge_view_count (Model Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_view_count_Lifecycle Management.png}
% \caption{Challenge view count (Lifecycle Management)}
% \label{fig:Challenge_view_count (Lifecycle Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_view_count_Infrastructure Management.png}
% \caption{Challenge view count (Infrastructure Management)}
% \label{fig:Challenge_view_count (Infrastructure Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_view_count_Deployment Management.png}
% \caption{Challenge view count (Deployment Management)}
% \label{fig:Challenge_view_count (Deployment Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_view_count_Report Management.png}
% \caption{Challenge view count (Report Management)}
% \label{fig:Challenge_view_count (Report Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_view_count_Security Management.png}
% \caption{Challenge view count (Security Management)}
% \label{fig:Challenge_view_count (Security Management)}
% \end{figure}

% Thirdly, we visualize the favorite count evolution trend (using LOWESS) and three-sigma confidence bound ($\alpha$=0.003) for each macro topic on a monthly frequency. Figure~\ref{fig:Challenge_favorite_count (Code Management)} shows the evolution of challenge favorite count in \texttt{Code Management}. Figure~\ref{fig:Challenge_favorite_count (Data Management)} shows the evolution of challenge favorite count in \texttt{Data Management}. Figure~\ref{fig:Challenge_favorite_count (Model Management)} shows the evolution of challenge favorite count in \texttt{Model Management}. Figure~\ref{fig:Challenge_favorite_count (Lifecycle Management)} shows the evolution of challenge favorite count in \texttt{Lifecycle Management}. Figure~\ref{fig:Challenge_favorite_count (Infrastructure Management)} shows the evolution of challenge favorite count in \texttt{Infrastructure Management}. Figure~\ref{fig:Challenge_favorite_count (Deployment Management)} shows the evolution of challenge favorite count in \texttt{Deployment Management}. Figure~\ref{fig:Challenge_favorite_count (Report Management)} shows the evolution of challenge favorite count in \texttt{Report Management}. Figure~\ref{fig:Challenge_favorite_count (Security Management)} shows the evolution of challenge favorite count in \texttt{Security Management}. TODO:

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_favorite_count_Code Management.png}
% \caption{Challenge favorite count (Code Management)}
% \label{fig:Challenge_favorite_count (Code Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_favorite_count_Data Management.png}
% \caption{Challenge favorite count (Data Management)}
% \label{fig:Challenge_favorite_count (Data Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_favorite_count_Model Management.png}
% \caption{Challenge favorite count (Model Management)}
% \label{fig:Challenge_favorite_count (Model Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_favorite_count_Lifecycle Management.png}
% \caption{Challenge favorite count (Lifecycle Management)}
% \label{fig:Challenge_favorite_count (Lifecycle Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_favorite_count_Infrastructure Management.png}
% \caption{Challenge favorite count (Infrastructure Management)}
% \label{fig:Challenge_favorite_count (Infrastructure Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_favorite_count_Deployment Management.png}
% \caption{Challenge favorite count (Deployment Management)}
% \label{fig:Challenge_favorite_count (Deployment Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_favorite_count_Report Management.png}
% \caption{Challenge favorite count (Report Management)}
% \label{fig:Challenge_favorite_count (Report Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_favorite_count_Security Management.png}
% \caption{Challenge favorite count (Security Management)}
% \label{fig:Challenge_favorite_count (Security Management)}
% \end{figure}

% Fourthly, we visualize the participation count evolution trend (using LOWESS) and three-sigma confidence bound ($\alpha$=0.003) for each macro topic on a monthly frequency. Figure~\ref{fig:Challenge_participation_count (Code Management)} shows the evolution of challenge participation count in \texttt{Code Management}. Figure~\ref{fig:Challenge_participation_count (Data Management)} shows the evolution of challenge participation count in \texttt{Data Management}. Figure~\ref{fig:Challenge_participation_count (Model Management)} shows the evolution of challenge participation count in \texttt{Model Management}. Figure~\ref{fig:Challenge_participation_count (Lifecycle Management)} shows the evolution of challenge participation count in \texttt{Lifecycle Management}. Figure~\ref{fig:Challenge_participation_count (Infrastructure Management)} shows the evolution of challenge participation count in \texttt{Infrastructure Management}. Figure~\ref{fig:Challenge_participation_count (Deployment Management)} shows the evolution of challenge participation count in \texttt{Deployment Management}. Figure~\ref{fig:Challenge_participation_count (Report Management)} shows the evolution of challenge participation count in \texttt{Report Management}. Figure~\ref{fig:Challenge_participation_count (Security Management)} shows the evolution of challenge participation count in \texttt{Security Management}. TODO:

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_participation_count_Code Management.png}
% \caption{Challenge participation count (Code Management)}
% \label{fig:Challenge_participation_count (Code Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_participation_count_Data Management.png}
% \caption{Challenge participation count (Data Management)}
% \label{fig:Challenge_participation_count (Data Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_participation_count_Model Management.png}
% \caption{Challenge participation count (Model Management)}
% \label{fig:Challenge_participation_count (Model Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_participation_count_Lifecycle Management.png}
% \caption{Challenge participation count (Lifecycle Management)}
% \label{fig:Challenge_participation_count (Lifecycle Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_participation_count_Infrastructure Management.png}
% \caption{Challenge participation count (Infrastructure Management)}
% \label{fig:Challenge_participation_count (Infrastructure Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_participation_count_Deployment Management.png}
% \caption{Challenge participation count (Deployment Management)}
% \label{fig:Challenge_participation_count (Deployment Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_participation_count_Report Management.png}
% \caption{Challenge participation count (Report Management)}
% \label{fig:Challenge_participation_count (Report Management)}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\columnwidth]{figures/Evolution/Challenge_participation_count_Security Management.png}
% \caption{Challenge participation count (Security Management)}
% \label{fig:Challenge_participation_count (Security Management)}
% \end{figure}



% Machine learning (ML) is changing technology and creating innovations in areas like autopilot. However, many companies struggle to adopt these new technologies. For example, while a 2018 Gartner survey predicted that 23\% of large companies would use artificial intelligence (AI) in one year, only 5\% actually did by 2019~\footnote{\url{https://www.gartner.com/en/documents/4000966}}. This shows the challenges companies face in adding AI to their systems, given the regular updates and the difference between lab tests and real-world use. This is where machine learning operations (MLOps) come in. MLOps offers tools to effectively manage AI projects. Unlike regular software, ML systems can behave unpredictably, requiring special tests. Managing everything, from data collection to final deployment, is essential for ML systems to work well.

% in this framework, an ML asset is not limited to the model alone. It includes raw and refined datasets, scripts for feature engineering, hyperparameters of the model, configurations for training, evaluation metrics, deployment settings, and more. Each of these assets has its lifecycle, intricacies, and dependencies, making its management an intricate task. However, as the ML community delves deeper into building more sophisticated models and systems, managing these assets poses substantial challenges. The mutable nature of data, the iterative refinement of models, the evolving computational infrastructure, and the dynamic requirements of real-world applications introduce variabilities that can be daunting to handle~\cite{sculley2015hidden}. Additionally, the collaborative nature of ML projects, often involving interdisciplinary teams, increases the need for transparent, efficient, and robust asset management systems~\cite{sambasivan2021everyone}.

% Navigating the complexities of asset management during the machine learning lifecycle poses formidable challenges, especially in the MLOps framework, dedicated to optimizing the deployment and maintenance of ML systems~\cite{10.1145/3533378}. The iterative character of model development introduces a dynamic tension between the promotion of advancements and the maintenance of reproducibility. This landscape is further complicated by unpredictable data shifts, the need for meticulous configuration management, and the absence of standardized methodologies and tools. While platforms like MLflow offer some respite, the constantly evolving tech realm necessitates perpetual adaptation of asset management tools. The spectrum of responsibilities, from data and model versioning to parameter tuning, highlights the intricate task of managing ML assets. Despite various efforts, achieving consistent versioning, reproducibility, traceability, and collaboration remains an intricate puzzle for many practitioners.

% In our study, we observe certain open posts that provided both the root cause and potential resolution. To ensure internal validity, we opt to exclude these posts from our analysis. Although these posts are informative, the lack of closure means that we cannot conclusively verify the effectiveness of the suggested solutions through community feedback. As a result, we have chosen not to include a closed-loop analysis for these specific posts.


%Manual selection of tags and keywords to identify posts related to the management of ML assets can vary depending on individual judgment. To alleviate this concern, we iteratively refine our filtering criteria, continuously testing and adjusting the tags and keywords until the collected posts are consistent with the curated tools.

% In culmination, the intertwined evolution of the ML lifecycle, MLOps, and ML asset management showcases the dynamism of the ML field. As these systems mature, they collectively shape the future trajectory of machine learning, driving both its potential and its challenges. Similarly to the studies above, our research resonates with the underpinning idea that managing ML assets presents distinct challenges, as evidenced by Sculley et al.~\cite{sculley2015hidden}, Idowu et al.~\cite{idowu2021asset}, and Alshangiti et al.~\cite{Alshangiti2019WhyID}. Like them, we recognize the tangible complications of integrating ML into broader software and data ecosystems. However, our emphasis diverges as we concentrate solely on ML asset management in the MLOps framework. Through this lens, we reveal intricate insights into the challenges associated with the lifecycle of ML assets, the evolution of such assets, and the prevalent trends in version control. In contrast to the above studies, our methodology and approach stand out. Instead of a broad-spectrum analysis of challenges in ML application development or a general analysis of ML-related Stack Overflow queries, our study zeros in on asset management discussions across multiple platforms, including Stack Overflow, GitHub Issues, and tool-specific forums. To the best of our knowledge, our study is a pioneering effort that synthesizes such a multifaceted analysis to understand the real-world intricacies faced in ML asset management.

==> sections/x-rq2-results.tex <==
\section{RQ2 Result: Difficulty of Challenge Topics}
\label{sec:rq2-results}

In RQ2, we aim to identify the macro-topics in the collected posts that either have a higher unresolved rate or take an extended period to resolve. By analyzing these unresolved rates, we can pinpoint the areas of concern and focus on developing targeted solutions to effectively address these persistent issues. The insights derived from our findings are instrumental in prioritizing resources and efforts for ML practitioners.

\subsection{Difficulty of posts based on type of inquiry}

We examine the unresolved rate of the ML asset management posts and find that $63.97\%$ of the posts remain unresolved. This percentage suggests that ML asset management poses more challenges compared to other areas of software engineering. For context, the unresolved rate for non-deployment deep learning (DL) is $62.7\%$~\cite{chen2020comprehensive}, big data is $60.5\%$~\cite{bagherzadeh2019going}, mobile development at $55.0\%$~\cite{rosen2016mobile}, release engineering at $49.8\%$~\cite{openja2020analysis}, and concurrency development at $43.8\%$~\cite{Ahmed2018WhatDC}. Furthermore, our observations indicate that the median resolution time for all posts in ML asset management is $42.21$ hours. This duration is significantly longer than the resolution times observed in other software engineering domains. For comparison, the median resolution time for DL deployment/non-deployment is $6.75/2.43$ hours~\cite{chen2020comprehensive}, big data $3.30$ hours~\cite{bagherzadeh2019going}, release engineering $3.00$ hours~\cite{openja2020analysis}, mobile development $0.92$ hours~\cite{rosen2016mobile}, and concurrency development $0.70$ hours~\cite{Ahmed2018WhatDC}.

We further analyze at the inquiry type level and find that \textbf{knowledge inquiries have an unresolved rate of $65.56\%$, a figure slightly above the $62.85\%$ noted for problem inquiries}, as presented in Table~\ref{rq1:inquiry metrics}. We conduct Chi-square tests to confirm whether there is a significant difference in the unresolved rate distribution between two types of inquiry across (macro-)topics. The results, with two p-values of $1.0$, suggest that there are no significant differences in the unresolved rate distribution between knowledge and problem inquiries across (macro-)topics. 

\begin{table}
\centering
\caption{Prevelance and difficulty metrics based on inquiry type.}
\begin{tabular}{llll}
\toprule
Inquiry Type & Prevalence (\%) & Unresolved Rate (\%) & Median Resolution Time (h) \\
\midrule
Knowledge & 40.59 & 65.56 & 21.14 \\
Problem & 59.41 & 62.85 & 65.51 \\
\bottomrule
\end{tabular}
\label{rq1:inquiry metrics}
\end{table}

Our analysis of the collected posts reveals \textbf{a significant difference in the resolution time between problem and knowledge inquiries}, as illustrated in Table~\ref{rq1:inquiry metrics}. Specifically, \textbf{problem inquiries have a median resolution time of $65.51$ hours.} In contrast, \textbf{knowledge inquiries are resolved in a median time of $21.14$ hours.} Figure~\ref{rq2:resolution time} offers a more granular view of this disparity, showcasing the distribution of resolution times across various macro-topics on a logarithmic scale. This visualization confirms that, across numerous macro-topics, problem inquiries generally require a longer resolution time than knowledge inquiries. To validate our observation, we employ the Mann-Whitney U test, a nonparametric statistical method designed to compare differences between two independent samples, especially when the sample distributions are not normally distributed and the sample sizes are small~\cite{mann1947test}. Applying this test to all resolved posts, we find a significant difference between the two types of inquiry ($p=0.000$). To measure the magnitude of this difference, we use eta-squared, a measure of the size of the effect that quantifies the proportion of variance associated with each main effect and interaction effect~\cite{richardson2011eta}. We use the following rules of thumb to interpret the values for the eta-squared estimator: an effect size of $0.01$ is considered small, $0.06$ is medium, and $0.14$ or greater indicates a large effect size~\cite{cohen2013applied}. Our findings, quantified by the eta-squared value, reveal a relatively weak relationship, with a value of $0.027$.

Exploring further, we conduct Mann-Whitney U tests for each macro-topic between the two types of inquiry. The results show that \textbf{62.50\% (10 out of 16) of the macro-topics have significant differences in resolution time at a significance level of $0.05$.} The strength of association in these topics varied, with eta-squared values ranging from modest $0.016$ to more pronounced $0.065$. In these specific macro-topics, problem inquiries consistently take longer to resolve than knowledge inquiries. For clarity, Figure~\ref{rq2:resolution time} highlights the macro-topics with significant differences by marking them in bold. Understanding the content and purpose of these inquiries offers further insight to ML practitioners. Users who post knowledge inquiries typically look to broaden their understanding. They may be new to the domain or tool and seek specific guidance. Once these users have obtained the domain-specific information necessary, they can address similar questions afterwards on their own. However, those who post problem inquiries probably have a decent grasp of the domain but face more complex issues that domain-specific knowledge alone cannot resolve. %Problem inquiries, often centered on software abnormalities, inherently pose more complex and intricate challenges. They require diagnostic procedures to unravel unforeseen issues, which could be influenced by a multitude of variables and undetermined factors. On the other hand, knowledge inquiries, primarily seeking clarity on tool usage, comparisons, or best practices, are often addressing established facts or pre-documented guidelines, making them inherently more straightforward to resolve.

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{figures/RQ2/Macro-topic resolution time boxplot.pdf}
\caption{Distribution of resolution time (h) in logarithmic scale of each macro-topic for each inquiry type.}
\label{rq2:resolution time}
\end{figure}

\subsection{Difficulty of posts based on macro-topics}

\textbf{User Interface Management ($\hat{C}_{16}$) exhibits the highest unresolved rate at $71.43\%$ among all macro-topics}, as illustrated in Table~\ref{rq1:macro-topic list}. Despite the user interface inquiries that constitute a mere $1.36\%$ of all questions, they appear to be particularly difficult to resolve. These complexities might arise from the multifaceted challenges associated with designing, implementing and optimizing user interfaces, which include usability, accessibility, technical and aesthetic considerations~\cite{kim2021accessible}. This scenario underscores the pressing need for more comprehensive support for inquiries related to the user interface and visualization. Furthermore, \textbf{Data Development ($\hat{C}{04}$) and Model Deployment ($\hat{C}{09}$) rank as the second and third most challenging topics, with unresolved rates of $70.31\%$ and $67.63\%$ respectively.} Data development, which includes the creation and refinement of training datasets, can be intricate and laden with potential challenges~\cite{liang2022advances,sambasivan2021everyone}. Meanwhile, the configuration of model deployment demands a deep understanding, which might not come naturally to many ML practitioners. This underscores the potential demand for more intuitive, user-friendly tools, or in-depth tutorials to simplify model deployment processes.

Lastly, \textbf{with a $55.38\%$ unresolved rate, Code Management ($\hat{C}_{01}$) is identified as the least challenging macro-topic.} The prevalence of well-established tools, such as Git and Mercurial, suggests that a wealth of resources and solutions are readily available, which could make addressing related issues more straightforward.

The results and implications slightly change when we examine the median resolution time across macro-topics. Table~\ref{rq1:macro-topic list} shows that \textbf{Experiment Management ($\hat{C}_{07}$) has the longest median resolution time ($87.25$ h) across all macro-topics.} This contrasts with the previous conclusion that it has a low unresolved rate ($55.52\%$). This discrepancy suggests that, while questions on this topic are eventually addressed, they may require a longer deliberation or more expertise, pointing to a potential knowledge gap in the community. We also find that \textbf{Code Management ($\hat{C}_{02}$) and Observability Management ($\hat{C}_{13}$) are the second ($83.57$ h) and third ($64.07$ h) most difficult topics in terms of median resolution time.} This implies that managing source code and monitoring systems is a particularly challenging task in ML asset management. This may be due to the complexity of integrating multiple tools and services, dealing with large amounts of data, and the need for real-time monitoring and feedback. These challenges require specialized skills and knowledge, and it takes time for teams to resolve problems and optimize processes. 

In our findings, Security Management ($\hat{C}_{15}$) stands out with the shortest median resolution time at $18.09$ hours among all macro-topics. Yet, intriguingly, it also exhibits a high unresolved rate of 67.40\%. This discrepancy might suggest that while certain experts can quickly address security-related issues, the larger community faces challenges in understanding fundamental concepts or adhering to best practices in the security domain~\cite{paleyes2022challenges,sarker2020cybersecurity}. This underscores the need to democratize expert knowledge and potentially points toward the need for better educational resources and training in this domain.

\textbf{The analysis reveals significant differences in the resolution time for user inquiries across different (macro-)topics.} These disparities are statistically validated, underscored by a p-value of $0.002$ for macro-topics and an even more notable $0.000$ for topics, confirming the significant variance in resolution time. The associated eta-squareds - $0.039$ for macrotopics and $0.010$ for topics - although indicating a minor effect size, further highlight the nuanced differences in the data. In contrast, when assessing the unresolved rate using Chi-square tests, both the macro-topic and topic levels demonstrate a consistent lack of significant variation, as evidenced by matching p-values of $1.0$ for each.

The analysis reveals correlations between certain inquiry attributes and the resolution time. Specifically, \textbf{Kendall's tau test shows a slight positive correlation with a tau value of $0.145$ between the average number of links in the inquiries and the median resolution time at the topic level, with a significant p-value of $0.014$.} This suggests that inquiries with more links tend to have a longer resolution time. Furthermore, the relationship becomes more pronounced when considering the average number of code lines (LOC) in the inquiries. \textbf{A more robust positive correlation, characterized by a tau value of $0.210$, is observed between the LOC and the median resolution time for the topics.} The associated p-value of $0.000$ underscores the statistical significance of this finding. Previous studies~\cite{yazdaninia2021characterization,calefato2018ask,bhat2014min} have consistently associated the number of lines of code (LOC) and the number of links with the complexity of user inquiries. These elements are considered reflective indicators of the expected effort and duration necessary for effective resolution. For inquiries with many links, the complexity comes from the issues being connected to each other, requiring a broad approach to solve. Inquiries with a lot of code indicate complex coding issues that need in-depth analysis and strong programming knowledge to resolve. However, the causal relationship between the number of links or code lines and the increase in resolution times is unclear. More research is required to understand how these factors specifically influence the time needed to address complex inquiries.

Similarly, \textbf{we find a negative correlation with a tau value of $-0.383$ ($p=0.041$) between the resolution time and the unresolved rate of user inquiries across macro-topics} through analysis with Kendall's tau test. This suggests that as the resolution time decreases, there is a tendency for the unresolved rate to also decrease, though it is essential to note that the relationship is moderate. Delving deeper into the topic level, we find a consistency in this trend. Although it shows a weaker connection with a tau value of $-0.169$, there is still a borderline negative correlation supported by a p-value of $0.004$. These results reveal an interesting dynamic: \textbf{specific (macro-)topics, although characterized by a higher incidence of unresolved inquiries, experience accelerated resolutions once effective solutions are identified.} This pattern aligns with our earlier findings, where some macro-topics, such as Security Management ($\hat{C}_{15}$) display reversed rankings when assessed through two different difficulty metrics. Therefore, the complexity of inquiries might not be uniform across different macro-topics, and certain macro-topics, while having a higher volume of unresolved inquiries, can be resolved more quickly once effective resolutions are identified. However, there is a gap in our understanding of the evolution of these topics and the resolution of inquiries associated with them. It is plausible that recent technical advancements have led to a decrease in resolution time for certain topics of inquiry, contributing to the observed pattern. These breakthroughs could help resolve easier problems more efficiently, while more complex issues remain unresolved until the new techniques mature. There is a need for more in-depth research to explore this hypothesis. Answering these questions is crucial to develop targeted strategies to enhance the efficiency and effectiveness of problem resolution across various topics.

\begin{footnotesize}
\begin{mybox}{Summary of RQ2}
% \textbf{RQ header/name}
% \tcblower
\begin{itemize}
    \item Inquiries related to machine learning asset management have a higher unresolved rate ($63.97\%$) and a longer median resolution time ($42.21 h$) compared to other subjects in software engineering, such as non-deployment deep learning, big data, release engineering, mobile, and concurrency development. This suggests that issues in ML asset management are more complex or challenging to address than those in the mentioned areas.
    % \item For machine learning asset management posts, there is no significant difference in unresolved rates between problem and knowledge inquiries at a significance level of 0.05.
    % \item The resolution of issues from problem inquiries takes significantly more time than knowledge inquiries in 62.50\% of the topics, also at a significance level of 0.05.
    \item User Interface Management ($71.43\%$), Data Development ($70.31\%$), and Model Deployment ($67.63\%$) have the highest unresolved rate, while Experiment Management ($87.25$ h), Code Management ($83.57$ h) and Observability Management ($64.07$ h) have the longest median resolution time in posts related to ML asset management, indicating that these areas present the most persistent challenges for users and require a longer time for the community or support teams to address, suggesting the need for improved solutions, documentation, or user support in these domains. 
    \item Despite a consistent unresolved rate of user inquiries across topics at a significance level of $0.05$, the resolution time for inquiries differs significantly between topics at the same level, indicating that certain topics may inherently be more complex or require specialized knowledge to address, leading to different response times.
\end{itemize}
\end{mybox}
\end{footnotesize}
